Differentially Private Federated Learning on Heterogeneous Data

Federated Learning (FL) is a paradigm for large-scale distributed learning which faces two key challenges: (i) efficient training from highly heterogeneous user data, and (ii) protecting the privacy of participating users. In this work, we propose a novel FL approach (DP-SCAFFOLD) to tackle these two challenges together by incorporating Differential Privacy (DP) constraints into the popular SCAFFOLD algorithm. We focus on the challenging setting where users communicate with a "honest-but-curious" server without any trusted intermediary, which requires to ensure privacy not only towards a third-party with access to the final model but also towards the server who observes all user communications. Using advanced results from DP theory, we establish the convergence of our algorithm for convex and non-convex objectives. Our analysis clearly highlights the privacy-utility trade-off under data heterogeneity, and demonstrates the superiority of DP-SCAFFOLD over the state-of-the-art algorithm DP-FedAvg when the number of local updates and the level of heterogeneity grow. Our numerical results confirm our analysis and show that DP-SCAFFOLD provides significant gains in practice.

==> all_appendices_old.tex <==
\clearpage
\appendix
\onecolumn
\aistatstitle{Differentially Private Federated Learning on Heterogeneous Data\\{\large Supplementary Material}}
% \setcounter{section}{0} # TODO use letter for section

\section*{Organization of the Appendix}

This appendix is organized as follows. Appendix~\ref{app:complementary} summarizes the main notations and provide the detailed \dpfedavg for completeness.
Appendix~\ref{appendix:privacy} provides details on our privacy analysis. Appendix~\ref{app:othertheoreticalresults} gives the full proofs of our utility results for the convex, strongly-convex and nonconvex cases. Finally, Appendix~\ref{app:exp_all} provides more details on the experiments of Section~\ref{sec:experiments}, as well as additional results.

\section{Additional Information}
\label{app:complementary}

\subsection{Table of Notations}

Table~\ref{table_notations} summarizes the main notations used throughout the paper.

\begin{table}[h]
\caption{Summary of the main notations.} \label{table_notations}
\begin{center}
\begin{tabular}{ll}
\textbf{Symbol}  &\textbf{Description} \\
\hline \\
    $[n]$ & set $\{1,2,...,n\}$ for any  $n \in \mathbb{N}$\\
    $M$, $i \in [M]$ & number and index of users\\
    $T$, $t \in [T]$ & number and index of communication rounds\\
    $K$, $k \in [K]$ & number and index of local updates (for each user)\\
    $D_i$ & local dataset held by the $i$-th user, composed of points $d_1^i, \hdots, d^i_\r$\\
    $\r$ & size of any local dataset $D_i$\\
    $D$ & joint dataset ($\bigsqcup_{i=1}^{M} D_i$)\\
    $f_i(x,d)$ & loss of the $i$-th user for model $x$ on data record $d$ \\
    $F_i$ & local empirical risk function of the $i$-th user $(\frac{1}{\r}\sum_{j=1}^\r f_i(\cdot, d_j^i))$\\
    $F$ & global objective function $(\frac{1}{M}\sum_{i=1}^M F_i)$\\
    $x^t\in \mathbb{R}^d$ & server model after round $t$\\
    $y_i^k\in \mathbb{R}^d$ & model of $i$-th user after local update $k$ \\
    $c^t \in \mathbb{R}^d$ & server control variate after round $t$ \\
    $c_i^t\in \mathbb{R}^d$ & control variate of the $i$-th user after round $t$ \\
    $l\in (0,1)$ &  user sampling ratio\\ % at any round $t$\\
    $s\in (0,1)$ & data sampling ratio\\ % at any update $k$\\
    $\epsilon,\delta$ & differential privacy parameters \\
    $\sigma_g$ & standard deviation of Gaussian noise added for privacy\\
    $C$ & gradient clipping threshold\\
    $\beta$ & Lipschitz-smoothness constant\\
    $\mu$ & strong convexity parameter \\
    $\sigmaoracle^2$ & variance of stochastic gradients\\
    \hline
\end{tabular}
\end{center}
\end{table}








\subsection{\dpfedavg Algorithm}
The code of \dpfedavg is given in Algorithm~\ref{algo_dp_fedavg}.

% \begin{restatable}[t]{algorithm}{HBK}
 \begin{algorithm}
\DontPrintSemicolon
\caption{DP-FedAvg$(T,K,l,s,\sigma_g,C)$ \label{algo_dp_fedavg}}
  \KwInputServer{initial $x^0$}
  \KwOutput{$x^T$}
  \For{$t=1,...,T$}
    {
        \HiLiRed\textbf{User subsampling by the server:} $C^t \subset [M]$\\
        \textbf{Server communicates} $x^{t-1}$ to users $i \in C^t$\\
        \For{user $i \in C^t$}
        {
            Initialize model: $y_i^0 \leftarrow x^t$\\
            \For{$k=1,...,K$}
            {   
                \HiLiRed\textbf{Data subsampling by user: }$S_i^k \subset D_i$\\
                \For{sample $j \in S_i^k$}
                {
                    \textbf{Compute gradient:} $g_{ij} \leftarrow \nabla f_i(y_i^{k-1},d^i_{j}) $\\
                    \HiLiYellow \textbf{Clip gradient:} $\tilde{g}_{ij} \leftarrow g_{ij} / \max \big(1, ||g_{ij}||_2/C\big)$
                    }
                 \HiLiYellow\textbf{Add DP noise to local gradients:} $\tilde{H}_i^k \leftarrow \frac{1}{s \r}\sum_{j \in S_i^k} \tilde{g}_{ij} + \frac{2C}{s\r}\mathcal{N} (0,\sigma^2_g)$\\
                $y_i^{k} \leftarrow y_i^{k-1} - \eta_l \tilde{H}_i^k$}
            $\Delta y_i^t \leftarrow y_i^K - x^{t-1}$\\
            \textbf{User $i$ communicates to server:} $\Delta y_i^t$
            }
        \textbf{Server aggregates}: $\Delta x^t \leftarrow \frac{1}{lM}\sum_{i \in C^t}\Delta y_i^t$\ \\
        $x^{t} \leftarrow x^{t-1} + \eta_g\Delta x^t$
    }
 \end{algorithm}
% \end{restatable}

% \newpage
\section{Details on Privacy Analysis}
\label{appendix:privacy}

In this section, we provide the proof of our privacy results. We start by recalling standard results on differential privacy 
on composition and amplification by subsampling
in Section~\ref{formal_dp}.
Section~\ref{rdp_theory} reviews recent results in Rényi Differential Privacy (RDP) which allow to obtain tighter privacy bounds.
We then formally state and prove Claim~\ref{lemma_privacy} in Section~\ref{proof_claim}. Finally, we provide the proof of our main result (Theorem~\ref{theorem_privacy}) in Section~\ref{proof_theorem_privacy}.

\subsection{Reminders on Differential Privacy}
\label{formal_dp}

% \aurelien{there is no need to recall everything, only what you will actually need in the analysis. perhaps we can keep Lemma B.1, B.2 and the part on subsampling. The definition of privacy loss random variable is not used before B.2, so I suggest to move it there. the rest can be removed.}

In the following, we denote by %$f : \mathcal{X}^n \rightarrow \mathbb{R}^d$ (where $n,d \in \mathbb{N}^*$) refers to a real-valued query function,
$D \in \mathcal{X}^n$ to a dataset of size $n$. Two datasets $D,D' \in \mathcal{X}^n$ are said to be neighboring (denoted by $||D-D'||\leq 1$) if they differ in at most one element.
% to a neighboring dataset of $D$ (that is $||D-D'|| \leq 1)$.

% \paragraph{Details on Definition~\ref{definition_dp}.} 

% The classic definition of DP ensures that it is impossible for any adversary, under some given probability, to get individual information from the aggregation of data records (which means that \textit{individual information is collectively hidden}). Differential privacy has three major positive properties:
% \begin{itemize}
%     \item it is \textbf{immune to post-processing} (no function computed on the output of the mechanism would make it less private);
%     \item it is \textbf{robust to auxiliary knowledge} (even if the adversary knows all but one record, the guarantee is still relevant);
%     \item it is \textbf{robust under composition} (one can control the degradation of the privacy if several analyses with DP guarantees are performed on the same data, see Lemma \ref{lemma_strong_composition}).
% \end{itemize}

% In order to better express inequalities on the tails of distribution, the DP analysis of a mechanism $M$ often refers to the \textit{privacy loss random variable} \citep{dp_deep_l, renyi_dp_sampled_gm_explicit}. Let $M(D)$ and $M(D')$ be the probability distributions (discrete or continuous) inherited from $M$ respectively induced on $D$ and $D'$. Then the privacy loss $L^M_{D,D'}$ is defined as follows:
% \begin{align}
%     L^M_{D,D'}(\theta):=\log\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)}\bigg) \quad \text{where } \theta \sim M(D). \label{eq:privacy_loss}
% \end{align}
% The interpretation of this quantity is thus easy to understand: $(\epsilon, \delta)$-DP ensures that the absolute value of the privacy loss is bounded by $\epsilon$ with probability at least $(1-\delta)$ \citep[Lemma 3.17]{dp_foundations}.

% \paragraph{Sensitivity.} 

% In order to achieve DP on $f$ regarding Eq.~\eqref{eq:privacy_loss}, it is natural to consider an \textit{output perturbation}. It often results in \textit{adding} a noise calibrated to $\Delta f$, known as the \textit{sensitivity} of $f$, to $f(D)$. In this paper, we define $\Delta_2(f)$ as the $l_2$-sensitivity of $f$ such that: $\Delta_2(f)=\max_{||D-D'|| \leq 1}||f(D) -f(D')||_2$. Intuitively, it gives the scale of the uncertainty needed to hide the contribution of any individual record.

% \paragraph{Gaussian mechanism.} 

% Among all mechanisms introducing $(\epsilon, \delta)$-DP, the \textit{Gaussian mechanism} is one of those whose privacy loss is simple to quantify, which is the reason why it is often used in practice \citep{dp_erm, dp_deep_l, analytical_gm}. Plus, it has multiple advantages: (i) a sum of Gaussian random variables is Gaussian, which can be useful to compose mechanisms; (ii) we can easily characterize the tails of Gaussian distribution; (iii) it may be the same type as other sources of noise encountered in machine learning problems. Given $f$ and a privacy budget $(\epsilon, \delta)$, we define the corresponding Gaussian mechanism $G_f(D)$ as $G_f(D):= f(D) + \mathcal{N}(0, \Delta_2 (f)^2 \sigma_g^2 \text{I}_d)$ where $\sigma_g$ is expressed in Lemma \ref{lemma_gaussian_dp} (remark that this noise is unbiased).

% \begin{lemma}[\textbf{Gaussian mechanism \citep[Theorem~3.22]{dp_foundations}}] Let $(\epsilon_0, \delta_0)$ be a given privacy budget to perturb $f(D)$, where $\epsilon_0 \leq 1$. Suppose we set $\sigma_g$ such that: $ \sigma_g=\sqrt{2\log(1.25/\delta_0)}/\epsilon_0$.\label{lemma_gaussian_dp}

% Then (i) $G_f$ is $(\epsilon_0,\delta_0)$-DP w.r.t. $D$ and (ii) $G_f$ is unbiased and has bounded variance such that:
% \begin{center}
%     $\mathbb{E}[G_f(D)]=f(D) \quad$ and $\quad \mathbb{E}||G_f(D) - f(D) ||^2 = \displaystyle\frac{4d\Delta_2(f)^2 \log(1.25/\delta_0)}{\epsilon_0^2}$.
% \end{center}
% \end{lemma}

% \begin{proof}
% Statement (i) is a result of privacy established by \cite{dp_foundations}, which uses Gaussian concentration inequalities. The unbiasness is directly obtained from the definition stated above. The result on the variance comes from:
% \begin{align*}
%     \mathbb{E}||G_f(D) - f(D) ||^2& = \mathbb{E}||\mathcal{N}(0,\Delta_2(f)^2\sigma_g^2 \text{I}_d)||^2\\
%     & = \Delta_2(f)^2\sigma_g^2 \mathbb{E}||\mathcal{N}(0,\text{I}_d)||^2\\
%     & = 2d \Delta_2(f)^2 \sigma_g^2. && \text{(variance of $\chi^2_d$ law)}
% \end{align*}
% \end{proof}

\paragraph{Composition.}

% Composing one DP mechanism over several iterations, while reusing outputs of past iterations, naturally degrades its final privacy bound. One advantage of the DP framework is to quantify this privacy loss. 

Let $M_1(\cdot;A_1), ..., M_T(\cdot;A_T)$ be a sequence of $T$ \textit{adaptive} DP mechanisms where $A_t$ stands for the auxiliary input to the $t$-th mechanism, which may depend on the outputs of previous mechanisms $(M_{t'})_{t'<t}$. The ability to choose the sequences of mechanisms adaptively is crucial for the design of iterative machine learning algorithms.
% (remark that \textit{adaptive} mechanisms are coherent with machine learning framework where the same parameters are continually optimized over the iterations of the algorithms).
DP allows to keep track of the privacy guarantees when such a sequence of private mechanisms is run on the same dataset $D$. 
Simple composition \citep[Theorem III.1.]{boosting_dp} states that the privacy parameters grow linearly with $T$. \cite{boosting_dp} provide a \textit{strong composition} result where the $\epsilon$ parameter grows sublinearly with $T$. This result is restated in
Lemma~\ref{lemma_strong_composition}. 

\begin{lemma}[Strong Adaptive composition,
% \citep[Theorem III.3]{boosting_dp}
\citealp{boosting_dp}]
\label{lemma_strong_composition}
Let $M_1,...,M_T$ be $T$ adaptive $(\epsilon,\delta)$-DP mechanisms. Then, for any $\delta' >0$, the mechanism $M=(M_1,...,M_T)$ is $(\overline{\epsilon},\overline{\delta})$-DP where:
\begin{align*}
     \overline{\epsilon}=\epsilon \sqrt{2T\log(1/\delta')} + T\epsilon (e^{\epsilon} -1) \text{ and }\overline{\delta}=T\delta+ \delta'.
\end{align*}
\end{lemma}

\textbf{Remark.} When stating theoretical results, $\overline{\epsilon}$ is typically approximated by $\mathcal{O}(\epsilon\sqrt{T\log(1/\delta')})$ when $\epsilon < 1$.

\paragraph{Privacy amplification by subsampling.} 

A key result in DP is that applying a private algorithm on a random subsample of the dataset amplifies privacy guarantees \cite{dp_subsampling}. % The DP framework ensures to gain \textit{some privacy} if only a subset of the original dataset (\textit{randomly chosen}) is used as input for the query function $f$. We say that privacy is \textit{amplified by subsampling}. \cite{dp_subsampling} especially provide a result,
In this work, we are interested in subsampling without replacement.

\begin{definition}[Subsampling without replacement]
\label{def_subsampling}
The subsampling procedure $\text{Samp}_{n,m} : \mathcal{X}^{n} \rightarrow \mathcal{X}^{m}$ (where $m \in \mathbb{N}$, with $m \leq n$) takes $D$ as input and chooses uniformly among its elements a subset $\underline{D}$ of $m$ elements. We may also denote $\text{Samp}_{n,m}$ as $\text{Samp}_{q}$ where $q=m/n$ in the rest of the paper.
\end{definition}

Lemma \ref{lemma_subsampling}) quantifies the associated privacy amplification effect.
% with the procedure of subsampling described in Definition~\ref{def_subsampling}.

\begin{lemma}[Amplification by subsampling, \citealp{dp_subsampling}]
\label{lemma_subsampling}
Let $M' : \mathcal{X}^{m} \rightarrow \mathcal{Y}$ be a $(\epsilon,\delta)$-DP mechanism w.r.t a given dataset $\underline{D} \in \mathcal{X}^{m}$. Then, mechanism $M : \mathcal{X}^{n} \rightarrow \mathcal{Y}$ defined as $M:=M'\circ \text{Samp}_{n,m}$ is $(\epsilon', \delta')$-DP w.r.t. to any dataset $D \in \mathcal{X}^{n}$ such that $\underline{D}=\text{Samp}_{n,m}(D)$, where:
\begin{center}
    $\epsilon'=\log(1 + q(e^{\epsilon} -1))$, $\delta'=q\delta$, $q=m /n$.
\end{center}
\end{lemma}
\textbf{Remark.} In theoretical results, $\epsilon'$ is often approximated by $\mathcal{O}(q\epsilon)$ when $\epsilon\leq 1$.


\subsection{Rényi Differential Privacy}
\label{rdp_theory}

\cite{dp_deep_l} demonstrated in practice that the privacy bounds provided by standard $(\epsilon,\delta)$-DP theory (see Section~\ref{formal_dp}) often overestimate the actual privacy bound. % Their work aims at calculating with more precision the evolution of the privacy loss over the different procedures (for example, subsampling and composition) in SGD framework, by using the \textit{Moments Accountants Technique}.
In order to better express inequalities on the tails of the output distributions of private algorithms, we introduce 
% the DP analysis of a mechanism $M$ often refers to
the \textit{privacy loss random variable} \citep{dp_foundations,dp_deep_l, renyi_dp_sampled_gm_explicit}. Given a random mechanism $M$, let $M(D)$ and $M(D')$ be the distributions of the output when $M$ is run on $D$ and $D'$ respectively. The privacy loss $L^M_{D,D'}$ is defined as:
\begin{align}
    L^M_{D,D'}(\theta):=\log\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)}\bigg) \quad \text{where } \theta \sim M(D). \label{eq:privacy_loss}
\end{align}
The interpretation of this quantity is easy to understand: $(\epsilon, \delta)$-DP ensures that the absolute value of the privacy loss is bounded by $\epsilon$ with probability at least $(1-\delta)$ for all pairs of neighboring datasets $D$ and $D'$ \citep[Lemma 3.17]{dp_foundations}.

We will reason on the \textit{Cumulant Generating Function} (CGF) of the privacy loss, denoted $K_M$, rather than on the privacy loss $L^M$ itself.
% (which thus does not depend on the output of the mechanism $\theta$ anymore, but on a positive parameter $\lambda$).
This CGF is expressed as follows for any $\lambda>0$:
\begin{align*}
 K_M(D,D',\lambda)=\mathbb{E}_{\theta\sim M(D)}\big[e^{\lambda L^M_{D, D'}(\theta)}\big]= \mathbb{E}_{\theta\sim M(D)}\bigg[\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)} \bigg)^{\lambda}\bigg],
\end{align*}
which is also equivalent to:
\begin{align}
     K_M(D,D',\lambda)=\mathbb{E}_{\theta\sim M(D')}\bigg[\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)} \bigg)^{\lambda+1}\bigg]. \label{eq:cgf}
\end{align}

By the property of the moment generating function, $K_M(D,D',.)$ fully determines the distribution of the privacy loss random variable $L^M_{D, D'}$.
% (which why it is equivalent to work on the CGF or on the privacy loss).
We also define $K_M(\lambda):=\sup_{||D-D'||\leq 1} K_M(D,D',\lambda)$, which is the upper bound on the CGF for any pair of neighboring datasets.


We can now introduce \textit{Rényi Differential Privacy} (RDP), which generalizes DP using the Rényi divergence $D_{\alpha}$.

\begin{definition}[Rényi Differential Privacy, %\citep[Definition 4]{renyi_dp}
\citealp{renyi_dp}]\label{def_rdp} For any $\alpha \in (1,\infty)$ and any $\epsilon>0$, a mechanism $M :\mathcal{X}^n \rightarrow \mathcal{Y}$ is said to be $(\alpha, \epsilon)$-RDP, if for all neighboring datasets $D$ and $D'$,
\begin{align}
    D_\alpha(M(D)||M(D')):=\displaystyle\frac{1}{\alpha -1}\log \mathbb{E}_{\theta\sim M(D')}\bigg[\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)} \bigg)^{\alpha}\bigg] \leq \epsilon.\label{eq:rdp_inequality}
\end{align}
\end{definition}

Given a mechanism $M$ and a RDP parameter $\alpha$, we can thus determine from Definition~\ref{def_rdp} the lowest value of the $\epsilon$-RDP bound, denoted $\epsilon_M(\alpha)$, such that $M$ is $(\alpha, \epsilon_M(\alpha))$-RDP. Indeed, $\epsilon_M(\alpha)$ is such that:
\begin{align*}
    \epsilon_M(\alpha)= \inf_{\epsilon \in \varepsilon(M)} \epsilon \quad \text{where}\quad \varepsilon(M):=\{\epsilon>0 : \sup_{||D-D'||\leq 1} D_\alpha(M(D)||M(D')) \leq \epsilon\}.
\end{align*}

The obvious similarity between Eq.~\eqref{eq:cgf} and Eq.~\eqref{eq:rdp_inequality} shows the link between the CGF and the notion of RDP. Indeed, for any $\alpha \in (1,\infty)$, it is easy to see that $(\alpha-1)\epsilon_M(\alpha)$ is equal to $K_M(\lambda)$ where $\lambda+1=\alpha$ (restated in Lemma~\ref{lemma_conversion_rdp_cgf}).
\begin{lemma}[\textbf{Equivalence RDP-CGF}]\label{lemma_conversion_rdp_cgf} Any mechanism $M$ is $(\lambda +1, K_M(\lambda)/\lambda)$-RDP for all $\lambda >0$. 
\end{lemma}

% \paragraph{Remark.}For $\alpha = 1$, the Rényi divergence is defined by continuity and reduces to Kullback-Leibler divergence, that is:
% \begin{align}
%     D_1(M(D)||M(D'))=\mathbb{E}_{\theta\sim M(D)}\bigg[\log\bigg(\displaystyle\frac{M(D)(\theta)}{M(D')(\theta)}\bigg)\bigg]=\mathbb{E}_{\theta\sim M(D)}\big[L^M_{D,D'}(\theta)\big].\label{eq:kullback_leibler}
% \end{align}
% Using $1$-RDP would thus be equivalent to set a bound on the expectation of the privacy loss random variable (weaker than DP). 

We now recall how we can convert RDP guarantees into standard DP guarantees.

\begin{lemma}[RDP to DP conversion,
%\citep[Proposition 3]{renyi_dp}
\citealp{renyi_dp}]\label{lemma_conversion_rdp_dp} If $M$ is $(\epsilon, \alpha)$-RDP, then $M$ is $(\epsilon + \log(1/\delta)/(\alpha-1),\delta)$-DP for any $0<\delta<1$.
\end{lemma}

% From Lemma~\ref{lemma_conversion_rdp_dp}, we see that setting $\alpha \rightarrow \infty$ in RDP is equivalent to state a result $(\epsilon, 0)$-DP (stronger than $(\epsilon, \delta)$-DP where $\delta>0$). This remark along with Eq.~\eqref{eq:kullback_leibler} highlight very well how RDP generalizes DP.

Given Lemma~\ref{lemma_conversion_rdp_dp} and Lemma~\ref{lemma_conversion_rdp_cgf}, it is possible to find the smallest $\epsilon$ from some fixed parameter $\delta$ or the smallest $\delta$ from some fixed parameter $\epsilon$ so as to achieve $(\epsilon, \delta)$-DP:
\begin{align}
    % \delta \rightarrow \epsilon: &\quad
    \epsilon(\delta)&=\min_{\lambda>0}\displaystyle\frac{\log(1/\delta)+K_M(\lambda)}{\lambda}, \label{epsilon_pb}\\
    % \epsilon \rightarrow \delta:  & \quad
    \delta(\epsilon)&=\min_{\lambda>0}e^{K_M(\lambda)-\lambda\epsilon}.\label{delta_pb}
\end{align}

Moreover, $\lambda \rightarrow K_M(\lambda)/\lambda$ is monotonous \citep[Theorem 3]{property_rdp} and $\lambda \rightarrow K_M(\lambda)$ is convex \citep[Theorem 11]{property_rdp}. This last property enables to bound $K_M$ by a linear interpolation between the values of $K_M$ evaluated at integers, as stated below: 
\begin{align}
    \forall \lambda >0, K_{M}(\lambda) \leq (1-\lambda + \lfloor\lambda\rfloor)K_{M}(\lfloor\lambda\rfloor) + (\lambda - \lfloor\lambda\rfloor)K_{M}(\lceil\lambda\rceil).\label{eq:convexity_km}
\end{align}

Therefore, Problem~\eqref{epsilon_pb} is quasi-convex and Problem~\eqref{delta_pb} is log-convex, and both can be solved if we know the expression of $K_M(\lambda)$ for any $\lambda >0$.

We provide below other useful results from RDP theory, which we will use in our privacy analysis.

\begin{lemma}[RDP Composition,
% \citep[Proposition 1]{renyi_dp}}
\citealp{renyi_dp}]\label{lemma_composition_rdp} Let $\alpha \in (1, \infty)$. Let $M_1$ and $M_2$ be two mechanisms such that $M_1$ is $(\alpha, \epsilon_1)$-RDP and $M_2$, which takes the output of $M_1$ as auxiliary input, is $(\alpha, \epsilon_2)$-RDP. Then the composed mechanism $M_2\circ M_1$ is $(\alpha, \epsilon_1 + \epsilon_2)$-RDP.
\end{lemma}

\begin{lemma}[RDP Gaussian mechanism,
% \citep[Corollary 3]{renyi_dp}
\citealp{renyi_dp}] \label{lemma_rdp_gaussian} If $f : \mathcal{X}^n \rightarrow \mathbb{R}^d$ has $\ell_2$ sensitivity 1, then the Gaussian mechanism $G_f(\cdot):= f(\cdot) + \mathcal{N}(0, \sigma_g^2 \text{I}_d)$ is $(\alpha, \alpha/2\sigma_g^2)$-RDP for any $\alpha>1$. 
\end{lemma}

\begin{lemma}[RDP for subsampled Gaussian mechanism, %\citep[Theorem 9]{renyi_dp_sampled_gm_explicit}
\citealp{renyi_dp_sampled_gm_explicit}]\label{lemma_subsampling_rdp} Let $\alpha \in \mathbb{N}$ with $\alpha \geq 2$ and $0<q<1$ be a subsampling ratio. Suppose $f : \mathcal{X}^n \rightarrow \mathbb{R}^d$ has $\ell_2$ sensitivity equal to 1. Let $G'_f(\cdot):=G_f\circ\text{Samp}_q(\cdot)$ be a subsampled Gaussian mechanism. 
Then $G'_f$ is $(\alpha, \epsilon(\alpha, \sigma_g^2))$-RDP where 
\begin{align*}
     \epsilon'(\alpha, \sigma_g^2) \leq \displaystyle \frac{1}{\alpha-1}\log\bigg(1 +2q^2 \binom{\alpha}{2}\min \{2(e^{1/\sigma_g^2}-1), e^{1/\sigma_g^2}\} +\displaystyle\sum_{j=3}^\alpha 2q^j \binom{\alpha}{j}e^{j(j-1)/2\sigma_g^2}\bigg).
 \end{align*}
\end{lemma}

\textbf{Remark.} By considering $q=o(1)$, the dominant term in the upper bound of $\epsilon'(\alpha, \sigma_g^2)$ comes from the term of the sum of the order of $q^2$. In particular, when $\sigma_g^2$ is large (i.e. high privacy regime), the term $\min \{2(e^{1/\sigma_g^2}-1), e^{1/\sigma_g^2}\}$ simplifies to $2(e^{1/\sigma_g^2}-1) \leq 4/\sigma_g^2$. This thus simplifies the whole upper bound to $\mathcal{O}(\alpha q^2/\sigma_g^2)$.

\subsection{Proof of Claim~\ref{lemma_privacy}}
\label{proof_claim}

We restate below a more formal version of Claim~\ref{lemma_privacy} along with its proof. For any $t\in [T]$, we define \textit{subversions} of algorithms \texttt{DP-SCAFFOLD} (Alg.~\ref{algo_dp_scaffold}) and \texttt{DP-FedAvg} (Alg.~\ref{algo_dp_fedavg}), which stop at round $t$ and reveal an output, either to the server or to a third party:
\begin{itemize}
    \item \textbf{To the server.} We assume that the sampling of users $C^t$ is known by the server. Formally, we define $\mathcal{A}_{\dpscaf}^t$, which outputs (reveals) $\{y_i^t, c_i^t\}_{i \in C^t}$, and $\mathcal{A}_{\dpfedavg}^t$, which outputs $\{y_i^t\}_{i \in C^t}$ (those quantities being private w.r.t. $\{D_i\}_{i \in C^t}$).
    \item \textbf{To a third party.} We define $\mathcal{\tilde{A}}_{\dpscaf}^t$, which  outputs  $(x^t, c^t)$ and $\mathcal{\tilde{A}}_{\dpfedavg}^t$, which outputs $x^t$ (those quantities being private w.r.t. $D$).
\end{itemize}

In both privacy models, \texttt{DP-SCAFFOLD} and \texttt{DP-FedAvg} can be seen as $T$ adaptive compositions of these \textit{sub}-algorithms. 

\begin{claim}[Formal version of Claim~\ref{lemma_privacy}]\label{claim_privacy_complete} For any $t\in [T]$, the following holds:
\begin{itemize}
    \item $\mathcal{A}_{\dpscaf}^t$ and $\mathcal{A}_{\dpfedavg}^t$ have the same level of privacy (towards the server),
    \item $\mathcal{\tilde{A}}_{\dpscaf}^t$ and $\mathcal{\tilde{A}}_{\dpfedavg}^t$ have the same level of privacy (towards a third party).
\end{itemize}
\end{claim}

\begin{proof}
We prove the claim by reasoning by induction on the number of communication rounds $t$. We only give the proof for the first statement (including the \texttt{DP-SCAFFOLD-warm} version). The second one can be proved in a similar manner.

First, consider $t=1$. For any $i \in C^t$, control variates $c_i^0$ are either all set to 0 (\texttt{DP-SCAFFOLD}), or $c_i^0$ are at least as private as $y_i^1$ (\texttt{DP-SCAFFOLD-warm}). The level of privacy for $\mathcal{A}_{\dpscaf}^1$ is thus \textit{fully} determined by the level of privacy of $\{y_i^1\}_{i \in C^t}$, which is the same as $\mathcal{A}_{\dpfedavg}^1$. Therefore the claim is true for $t=1$.

Then, let $t \in [T]$ and suppose that the claim is verified for all $t'<t$.
Let $i\in C^t$ and first consider $\mathcal{A}_{\dpscaf}^t$. The update of the $i$-th user model (see Eq. \ref{eq:update_y_i}) at round $t$ shows that an additional information leakage may come from the correction $(c^{t-1} - c_i^{t-1})$ (actually from $c_i^{t-1}$ since $c^{t-1}$ is known by the server). By assumption of induction, $c_i^{t-1}$ is also known by the server. Therefore, using the post-processing property of DP, the $y_i^t$ as updated in \texttt{DP-SCAFFOLD} is as private w.r.t. $D_i$ as the $y_i^t$ as updated in \texttt{DP-FedAvg}. Besides this, the update of the $i$-th control variate \textit{fully} depends on the local updates of $y_i^t$ through the mean of the DP-noised stochastic gradients calculated over the local iterations. Therefore,  considering all the contributions from $C^t$, $\mathcal{A}_{\dpfedavg}^t$ and $\mathcal{A}_{\dpscaf}^t$ have the same level of privacy.
\end{proof}

\subsection{Proof of Theorem~\ref{theorem_privacy}}
\label{proof_theorem_privacy}

\paragraph{Preliminaries.}

Lemma~\ref{lemma_subsampling_rdp} only gives an upper bound of the RDP privacy for a subsampled Gaussian mechanism when $\alpha \in \mathbb{N}$ with $\alpha \geq 2$. However we will need to optimize our privacy bound w.r.t. $\alpha \in \mathbb{R}$ with $\alpha>1$. We thus use Lemma~\ref{lemma_conversion_rdp_cgf} and the convexity of the CGF (see Eq.~\ref{eq:convexity_km}) to generalize this upper bound to the following result.

Let $\alpha \in \mathbb{R}$ with $\alpha >1$. Under the same assumptions as in Lemma~\ref{lemma_subsampling_rdp}, $G'_f$ is $(\alpha, \epsilon''(\alpha, \sigma_g^2))$-RDP with
\begin{align}
\label{eq:comp_general_alpha}
    \epsilon''(\alpha, \sigma_g^2) \leq (1 - \alpha +\lfloor \alpha\rfloor)\frac{\lfloor\alpha\rfloor - 1}{\alpha - 1}\epsilon'(\lfloor\alpha\rfloor - 1, \sigma_g^2) + (\alpha - \lfloor \alpha \rfloor)\frac{\lceil\alpha\rceil - 1}{\alpha - 1}\epsilon'(\lceil\alpha\rceil - 1, \sigma_g^2),
\end{align}
where $\epsilon'(\cdot, \sigma_g^2)$ admits the upper bound given in Lemma~\ref{lemma_subsampling_rdp}.

\paragraph{Details of the proof.}

Our privacy analysis assumes that the query function has sensitivity 1, since the calibration of the Gaussian noise is locally adjusted in our algorithms with the constant $S=2C/s\r$ (see Section~\ref{dp_framework}). We simply denote by $G$ the Gaussian mechanism with variance $\sigma_g^2$, which is $(\alpha, \alpha/2\sigma_g^2)$-RDP (Lemma~\ref{lemma_rdp_gaussian}). Below, we first prove privacy guarantees towards a third-party observing only the final result, and then deduce the guarantees towards the honest-but-curious server.

\paragraph{Step 1: data subsampling.}

Let $t\in[T]$ be an arbitrary round.
We first provide an upper bound $\epsilon_a$ for the privacy loss \textit{after the aggregation} by the server of the $lM$ individual contributions (line~\ref{aggregation_step0} in Alg.~\ref{algo_dp_scaffold}) thanks to the local addition of noise.
% Those are made \textit{private} w.r.t. to the corresponding local datasets by locally adding DP noise. 

Let $i \in C^t$, $\alpha>1$. We denote by $\epsilon_i(\alpha)$ the $\alpha$-RDP budget (w.r.t. $D_i$) used to ``hide`` the individual contribution of the $i$-th user from the server. This contribution is the result of the composition of $K$ adaptative $s$-subsampled mechanisms $G$:
\begin{itemize}
    \item We first obtain an upper RDP bound for the $s$-subsampled mechanism with Lemma~\ref{lemma_subsampling_rdp}. Suppose first $\alpha\in \mathbb{N}$ and $\alpha\geq 2$, which is the case covered by Lemma~\ref{lemma_subsampling_rdp}. Under Assumption~\ref{ass:dplebvels}-(i) and Assumption~\ref{ass:dplebvels}-(iii), the resulting mechanism is $(\alpha, \mathcal{O}(s^2\alpha/\sigma_g^2))$-RDP. To extend this result to $\alpha > 1$, we use the result provided in \eqref{eq:comp_general_alpha}: by factoring by $s^2/\sigma_g^2$ in the upper bound of $\epsilon''(\alpha, \sigma_g^2)$, and bounding the rest of the inequality (a convex combination between $(\lfloor \alpha \rfloor -1)^2/(\alpha -1)$ and $(\lceil \alpha \rceil -1)^2/(\alpha -1)$) by $\alpha$, we also obtain that this mechanism is $(\alpha, \mathcal{O}(s^2\alpha/\sigma_g^2))$-RDP.
    \item We then use the result of Lemma~\ref{lemma_composition_rdp} for the RDP composition rule over the $K$ local iterations, which gives that $\epsilon_i(\alpha) \leq \mathcal{O}(Ks^2\alpha/\sigma_g^2)$.
\end{itemize}

We now consider the aggregation step. Taking into account all the contributions of the users from $C^t$, we get a Gaussian noise of variance $S^2\sigma_a^2$ where $\sigma_a^2=\frac{1}{lM}\sigma_g^2$. %Yet, making the whole aggregation private w.r.t. $D$ only requires a $l_2$ calibration equal to $S'=S/lM$ (by triangle inequality). By rewriting the variance $S^2\sigma_a^2$ as $S'^2 \times (lM\sigma_g^2)$, we prove that we save a factor $lM$ in the variance of the Gaussian noise to make the whole contribution private w.r.t. $D$.
Note that the sensitivity of the aggregation (w.r.t. the joint dataset $D$) is $lM$ times smaller than when considering an individual contribution. Therefore, with the previous approximation, the aggregated contributions satisfy $(\alpha, \mathcal{O}(Ks^2\alpha/lM\sigma_g^2))$-RDP w.r.t. $D$.

After converting this result into a DP bound (Lemma~\ref{lemma_conversion_rdp_dp}), we get that for any $0<\delta'<1$, the aggregation at line~\ref{aggregation_step0} in Alg.~\ref{algo_dp_scaffold} is $(\epsilon_a(\alpha, \delta'), \delta')$-DP w.r.t. $D$ where $\epsilon_a(\alpha, \delta')=\mathcal{O}\big(\frac{Ks^2\alpha}{lM\sigma_g^2} + \frac{\log(1/\delta')}{\alpha-1}\big)$. 

\textit{Without approximation:} we would obtain at this step an exact upper bound $\epsilon_a(\alpha, \delta')=K\epsilon''(\alpha,lM\sigma_g^2) + \frac{\log(1/\delta')}{\alpha-1}$.


\paragraph{Step 2: user subsampling.}

In order to get explicit bounds (which are slightly suboptimal), we then use classical DP tools to estimate an upper DP bound after $T$ rounds taking into account the amplification by subsampling from the set of users.

\begin{itemize}
    \item Using Lemma~\ref{lemma_subsampling}, the subsampling of users enables a gain of privacy of the order of $l$, which gives $\big(\mathcal{O}(l\epsilon_a(\alpha, \delta')), l\delta'\big)$-DP.
    \item Using Lemma~\ref{lemma_strong_composition}, we compose this mechanism over $T$ iterations, which under Assumption~\ref{ass:dplebvels}-(ii) gives for any $\delta''>0$, $\big(\mathcal{O}(\sqrt{T\log(1/\delta'')}l\epsilon_a(\alpha, \delta')), Tl\delta' + \delta''\big)$-DP.
\end{itemize}

\textit{Without approximation}: the mechanism is $\big(\epsilon^*(\alpha,\delta') \sqrt{2T\log(1/\delta'')} + T\epsilon^*(\alpha,\delta') (e^{\epsilon^*(\alpha,\delta')} -1), Tl\delta' + \delta''\big)$ where $\epsilon^*(\alpha,\delta')=\log(1 + l(e^{\epsilon_a(\alpha,\delta')} -1))$.


\paragraph{Step 3: setting parameters.}

We denote $\epsilon_T(\alpha,\delta',\delta'')=l\sqrt{T\log(1/\delta'')}\big(\frac{Ks^2\alpha}{lM\sigma_g^2} + \frac{\log(1/\delta')}{\alpha-1}\big)$. Given what is stated above, the final output of the algorithm is $(\mathcal{O}(\epsilon_T),Tl\delta' + \delta'')$-DP.

Considering our final privacy budget $\delta$, we \textit{arbitrarily} fix $\delta':=\delta/2Tl$ and $\delta'':=\delta/2$. We now aim to find an expression of $\sigma_g$ such that the privacy bound is minimized. \textit{By considering the approximated bound}, this gives the following minimization problem:
\begin{align*}
    \min_{\alpha >1} \epsilon_T(\alpha):=l\sqrt{T\log(2/\delta)}\bigg(\frac{Ks^2\alpha}{lM\sigma_g^2} + \frac{\log(2Tl/\delta)}{\alpha-1}\bigg).
\end{align*}
Using DP rather than RDP has the advantage to solve this minimization problem pretty easily since only the second factor in $\epsilon_T(\alpha)$ depends on $\alpha$, that is:
\begin{align*}
    \min_{\alpha >1} \tilde{\epsilon_T}(\alpha):=\frac{Ks^2\alpha}{lM\sigma_g^2} + \frac{\log(2Tl/\delta)}{\alpha-1}.
\end{align*}

By omitting constants, we obtain the expression for the minimum value of $\epsilon_T(\alpha)$:
\begin{align*}
    \tilde{\epsilon}=l\sqrt{T\log(2/\delta)}\bigg(\frac{s\sqrt{K\log(2Tl/\delta)}}{\sigma_g\sqrt{lM}}+\frac{Ks^2}{lM\sigma_g^2}\bigg).
\end{align*}
Under Assumption~\ref{ass:dplebvels}-(iii), we can bound the second term by the first one, which gives:
\begin{align*}
    \tilde{\epsilon}=\mathcal{O}\bigg(\frac{s\sqrt{lTK\log(2/\delta)\log(2Tl/\delta)}}{\sigma_g\sqrt{M}}\bigg).
\end{align*}
We then invert the formula of this upper bound of $\tilde{\epsilon}$ to express $\sigma_g$ as a function of a given privacy budget $\epsilon$:
\begin{align*}
     \sigma_g=\Omega\big(s\sqrt{lTK\log(2Tl/\delta)\log(2/\delta)}/\epsilon\sqrt{M}\big),
\end{align*}
which proves that the algorithm is $(\mathcal{O}(\epsilon),\delta)$-DP towards a third-party observing its final output.

\textit{Without approximation:} the minimization problem is much more complex and has to be solved numerically
\begin{align*}
    \min_{\alpha>1,\delta'>0,\delta''>0} \epsilon^*(\alpha,\delta') \sqrt{2T\log(1/\delta'')} + T\epsilon^*(\alpha,\delta') (e^{\epsilon^*(\alpha,\delta')} -1) \quad \text{s.t. } \delta=Tl\delta' + \delta',
\end{align*}
or:
\begin{align*}
    \min_{\alpha>1,x \in (0,1)} \epsilon^*(\alpha,x\delta/Tl) \sqrt{2T\log(1/(1-x)\delta)} + T\epsilon^*(\alpha,x\delta/Tl) (e^{\epsilon^*(\alpha,x\delta/Tl)} -1).
\end{align*}


\paragraph{Extension to privacy towards the server.} The crucial difference with the third-party case is that the server observes individual contributions and knows which users are subsampled at each step. Removing the privacy amplification effect of the $l$-subsampling of users and the aggregation step, the minimization problem becomes
\begin{align*}
    \min_{\alpha >1} \epsilon_T(\alpha):=\sqrt{T\log(2/\delta)}\bigg(\frac{Ks^2\alpha}{\sigma_g^2} + \frac{\log(2T/\delta)}{\alpha-1}\bigg),
\end{align*}
where the minimizing value can be approximated by:
\begin{align*}
    \tilde{\epsilon}=\sqrt{T\log(2/\delta)}\bigg(\frac{s\sqrt{K\log(2T/\delta)}}{\sigma_g}+\frac{Ks^2}{\sigma_g^2}\bigg).
\end{align*}

Under Assumption~\ref{ass:dplebvels}-(iii), we can bound the second term by the first one:
\begin{align*}
    \tilde{\epsilon}=\mathcal{O}\bigg(\frac{s\sqrt{TK\log(2/\delta)\log(2T/\delta)}}{\sigma_g}\bigg),
\end{align*}
which proves that we obtain $(\mathcal{O}(\epsilon_s), \delta_s)$-DP towards the server where  $\epsilon_s=\mathcal\epsilon\sqrt{\frac{M}{l}}$ and $\delta_s=\frac{\delta}{2}(\frac{1}{l} + 1)$.

\paragraph{Remark.} 

For privacy towards a third-party, it is actually possible to combine the subsampling ratios (user and data) to determine a bound upon the subsampling of data \textit{directly} from $D$ and thus to quantify a more precise gain in privacy \citep{fl_shuffle}. The difficulty in this setup is that this combined subsampling is \textit{not uniform overall}, which requires extending the proof of Lemma~\ref{lemma_subsampling} as done by \citet{fl_shuffle}.


\section{Proof of Utility}
\label{app:othertheoreticalresults}

In this section, we provide the proof of our utility results. We first establish in Section~\ref{subsec_utility_preliminaries} some preliminary results about the impact of DP noise over stochastic gradients. In Section~\ref{subsec_utility_dp_scaffold}, we provide the complete version of our utility result for \texttt{DP-SCAFFOLD-warm} (Theorem~\ref{theorem_utility_scaffold}), from which Theorem~\ref{utility_result} is an immediate corollary. We prove this theorem for convex local loss functions in Section~\ref{subsec_utility_dp_scaffold_convex} and non-convex loss functions in Section~\ref{subsec_utility_dp_scaffold_non_convex}. We finally state in Section~\ref{subsec_utility_dp_fedavg} our complete result for \texttt{DP-FedAvg} (Theorem~\ref{theorem_utility_fedavg}).

For any $C,\sigma_g>0$, we define $\Sigma_g(C) := 2C\sqrt{2d}\sigma_g/s\r$. We recall that we assume that $F$ is bounded from below by $F^*= F(x^*)$, for an $x^* \in \mathbb{R}^d$. 

\subsection{Preliminaries}
\label{subsec_utility_preliminaries}

\paragraph{Properties of DP-noised stochastic gradients.}

Let $i \in [M]$, $x \in \mathbb{R}^d$, $S_i \subset D_i$ and $C,\sigma_g>0$. Suppose Assumptions~\ref{ass:smooth_f_i} and \ref{ass:stoch_grad}.3 are verified (the last assumption ensures that the clipping on per-example local gradients with threshold $C$ is not effective). 

We below recall from Section~\ref{algo_description} the expression of $\tilde{H}_i(x)$, which is the noised version of the local gradient $H_i(x)$ of the $i$-th user over $S_i$ evaluated at $x$ (omitting index $k$):

\begin{equation*}
    \tilde{H}_i(x):= H_i(x) + \frac{2C}{s\r} \mathcal N (0,\sigma^2_g) \quad \text{where} \quad H_i(x):= \frac{1}{s \r}\sum_{d_j^i \in S_i}\nabla f_i(x, d^i_j).
\end{equation*}

We recall that the $l_2$-sensitivity of $H_i(x)$ w.r.t. $S_i$ is upper bounded by $2C/s\r$, which explains the scaling of the Gaussian noise in the expression of $\tilde{H}_i(x)$. Since the variance of $\mathcal{N}(0, \text{I}_d)$ is $2d$, the following statement holds directly:
\begin{align*}
    \mathbb{E}\big[\tilde{H}_i(x)\big]=H_i(x)
    \text{ and }\mathbb{E}\big[||\tilde{H}_i(x)- H_i(x)||^2\big] \leq
     \displaystyle\frac{8C^2d\sigma_g^2}{s^2\r^2}=\Sigma_g(C)^2. 
\end{align*}

By combining our utility assumptions with the result stated above, we can deduce the following lemma. First, 

\begin{lemma}[\textbf{Regularity of DP-noised stochastic gradients}]\label{lemma_reg_h_tilde}
Under Assumptions~\ref{ass:smooth_f_i} and \ref{ass:stoch_grad}, for any iteration $t \in [T], k\in [K]$,
\begin{enumerate}
    \item$\mathbb{E}_{S_i^k,\mathcal{N}(0, \text{I}_d)}\big[\tilde{H}_i^k(y_i^{k-1})|y_i^{k-1}\big]=\nabla F_i(y_i^{k-1})$,
    \item $\mathbb{E}_{S_i^k,\mathcal{N}(0, \text{I}_d)}\big[||\tilde{H}_i^k(y_i^{k-1}) - \nabla F_i(y_i^{k-1})||^2|y_i^{k-1}\big] \leq 
     \displaystyle\frac{\varsigma^2}{s\r} + \Sigma_g^2(C)$.
\end{enumerate}
\end{lemma}

The proof of Lemma~\ref{lemma_reg_h_tilde} is easily obtained by conditioning on the two sources of randomness which are \textbf{independent} (ie, mini-batch sampling and Gaussian noise) thus the variance is additive. This result can be seen as a \textit{degraded} version of Assumption~\ref{ass:stoch_grad} due to the local injection DP noise, a fact that we will strongly leverage to derive convergence rates.

We now enumerate several statements that will be used in the utility proof. First, Lemma~\ref{lemma_nesterov} enables to control $||\nabla F||^2$ with assumption of smoothness over the local loss functions. Second, Lemma~\ref{lemma_mean_variance} provides separation inequalities of mean and variance \cite[Lemma 4]{fl_scaffold}, which enables to state a result on quantities of interest in Corollary~\ref{corollary_noise}.

\begin{lemma}[Nesterov inequality] \label{lemma_nesterov} Suppose Assumption~\ref{ass:smooth_f_i} is verified and assume that for all $i \in [M]$, $F_i$ is convex. Then,
    \begin{align*}
        \forall x \in \mathbb{R}^d, ||\nabla F(x)||^2 \leq 2 \beta (F(x) -F^*).
    \end{align*}
\end{lemma}
\begin{proof} Let $x \in \mathbb{R}^d$.
\begin{align*}
    ||\nabla F(x)||^2 & = ||\nabla F(x) -\nabla F(x^*)||^2=||\frac{1}{M}\sum_{i=1}^M \nabla F_i(x) -\nabla F_i(x^*)||^2\\
    & \leq \frac{1}{M}\sum_{i=1}^M||\nabla F_i(x) -\nabla F_i(x^*)||^2 && \text{(Jensen inequality)}\\
    &\leq 2\beta (F(x) -F^*) && \text{\cite[Theorem 2.1.5]{nesterov2018lectures}}
\end{align*}
\end{proof}

\begin{lemma}[Separating mean and variance] Let $(A_1,...,A_n)$ be $n$ random variables in $\mathbb{R}^d$ \textbf{not necessarily independent}.\\
\label{lemma_mean_variance}
1. Suppose that their mean is  $\mathbb{E}[A_i]=a_i$ and their variance is uniformly bounded, i.e. for all $i\in [n]$,  $\mathbb{E}[||A_i - a_i||^2]\leq \sigma^2_A$. Then,
\begin{align*}\mathbb{E}\left\|\displaystyle\sum_{i=1}^n A_i\right\|^2 \leq \left\|\displaystyle\sum_{i=1}^n a_i\right\|^2 + n^2\sigma^2_A.
\end{align*}

2. Suppose that their conditional mean is $\mathbb{E}[A_i|A_{i-1},...A_1]=a_i$ and their variance is uniformly bounded, i.e. for all $i\in [n]$,  $\mathbb{E}[||A_i - a_i||^2]\leq \sigma^2_A$. Then,
\begin{align*}
    \mathbb{E}\left\|\displaystyle\sum_{i=1}^n A_i\right\|^2 \leq 2 \left\|\displaystyle\sum_{i=1}^n a_i\right\|^2 + 2n\sigma^2_A.
\end{align*}
\end{lemma}

\begin{corollary} 
\label{corollary_noise}
Let $t \in [T]$. In the following statements, the expectation is taken w.r.t.~the randomness from their local data sampling, from the Gaussian DP noise, conditionally to the users' sampling  $C^t$. 
% We denote $\mathcal{Y}(C^t)$ as the set of random variables $\{C^t, \{y_i^{k-1}\}_{i \in C^t, k \in[K]}\}$ (defined conditionally to a certain user sampling $C^t$).

\begin{itemize}
\item $ \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} (\tilde{H}_i^k (y_i^{k-1}) - \nabla F_i(y^i_{k-1}))\Big\|^2 \bigg | C^t, y_0 \right]     {\le} \frac{\Sigma_g^2(C) + \varsigma^2/s\r}{(KlM)} $
    \item $\mathbb{E}\bigg[\Big\|\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\tilde{H}_i^k (y_i^{k-1})\Big\|^2|C^t\bigg]\leq 2 \mathbb{E}\bigg[\Big\|\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\nabla F_i(y_i^{k-1}) \Big\|^2|C^t\bigg] + 2 \frac{\varsigma^2}{KlsM\r} + 2 \frac{\Sigma_g^2(C)}{KlM}$,
    \item $\mathbb{E}\bigg[\Big\|\displaystyle\frac{1}{lM}\sum_{i \in C^t}c_i^t - \mathbb E[c^t_i]\Big\|^2|C^t, y_0\bigg] \le 
    \frac{\Sigma_g^2(C) + \varsigma^2/s\r}{KlM} $
    % = \mathbb{E}\bigg[\Big\|\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\tilde{H}_i^k (y_i^{k-1})\Big\|^2|C^t, y_0\bigg]$,
    \item $\mathbb{E}||c^t||^2 \leq \displaystyle\frac{1}{M}\sum_{i=1}^M||\mathbb{E}[c_i^t]||^2 + \frac{\varsigma^2}{KlsM\r} + \frac{\Sigma_g^2(C)}{KlM}$.
\end{itemize}
\end{corollary}

\begin{proof}  To simplify the proof, we deliberately omit the index $t $ denoting the index of the communication round in the considered random variables. 
% and to write the conditional expectations w.r.t. $\mathcal{Y}(C^t)$ as $\mathbb{E}[.|\mathcal{Y}(C^t)]$.\\

\textbf{First and second inequality.} We define a random variable $A$ such as $A:=\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} A_{i,k}$, with $A_{i,k}:= \tilde{H}_i^k(y_i^{k-1})$. 
% We aim at applying Lemma~\ref{lemma_mean_variance} on $A$, conditionally to $\mathcal{Y}(C^t).$\\

From Lemma~\ref{lemma_reg_h_tilde}, we have  that  for all $i\in C^t, k\in [K]$: $\mathbb{E}[A_{i,k}|C^t]=\mathbb{E}[\tilde{H}_i^k(y_i^{k-1})|(C^t)]= \mathbb E [\nabla F_i(y_i^{k-1})|(C^t)]$. Furthermore, by Lemma~\ref{lemma_reg_h_tilde},  $\mathbb{E}\left[||\tilde{H}_i^k(y_i^{k-1}) - \nabla F_i(y_i^{k-1})]||^2\right]\leq \Sigma_g^2(C) + \varsigma^2/s\r $.
    % \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}

Furthermore, (a) for $i,j\in C^t$,  $\sum_{k\in K} A_{i,k}-\nabla F_i(y_i^{k-1})$ and $\sum_{k\in K} A_{j,k}-\nabla F_j(y_j^{k-1})$ are independent conditionally to $C^t, y_0$; (b) for any $i\in C^t$,  $(A_{i,k}-\nabla F_i(y_i^{k-1}))_{k\in [K]}$ is a martingale increment, i.e., $\mathbb E[A_{i,k}-\nabla F_i(y_i^{k-1})|\sigma(y^i_{k'}, A_{i,k'\in[k-1]})]=0$. 

Consequently:
\begin{align*}
    % \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} A_{i,k} - \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} \nabla F_i(y^i_{k-1})\Big\|^2 \bigg | C^t, y_0 \right] &
     \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} (A_{i,k} - \nabla F_i(y^i_{k-1}))\Big\|^2 \bigg | C^t, y_0 \right]     & \overset{(a)}{=} \frac{1}{(KlM)^2} \sum_{i \in C^t} \mathbb E\left[\Big\| \sum_{k \in [K]} (A_{i,k} - \nabla F_i(y^i_{k-1}))\Big\|^2 \bigg | C^t, y_0 \right] \\
    & \overset{(b)}{=} \frac{1}{(KlM)^2} \sum_{i \in C^t} \sum_{k \in [K]}  \mathbb E\left[\Big\| (A_{i,k} - \nabla F_i(y^i_{k-1}))\Big\|^2 \bigg | C^t, y_0 \right] \\
    &{\le} \frac{\Sigma_g^2(C) + \varsigma^2/s\r}{(KlM)} .
\end{align*}






% we want to bound $\mathbb{E}||A- \mathbb{E}[A]||^2 = \mathbb{E}||\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\tilde{H}_i^k(y_i^{k-1}) - \nabla F_i(y_i^{k-1})]||^2$.  We have:

% \maxence{Le calcul ci dessous est faux}
% \begin{align*}
%     \mathbb{E}||A- \mathbb{E}[A]||^2 & \leq \displaystyle\frac{1}{(KlM)^2}\sum_{i \in C^t}\sum_{k \in [K]}\underbrace{\mathbb{E}||\tilde{H}_i^k(y_i^{k-1}) - \nabla F_i(y_i^{k-1})]||^2}_{\leq \Sigma_g^2(C) + \varsigma^2/s\r \text{ (Lemma~\ref{lemma_reg_h_tilde})}}\\
%     & \leq \displaystyle\frac{\Sigma_g^2(C) + \varsigma^2/s\r}{KlM}.
% \end{align*}

We also have that:
\begin{align*}
\mathbb E\left[\Big\| A \Big\|^2 \bigg | C^t, y_0 \right] \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} A_{i,k} \Big\|^2 \bigg | C^t, y_0 \right] & \le 2  \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} (A_{i,k} - \nabla F_i(y^i_{k-1}))\Big\|^2 \bigg | C^t, y_0 \right]   
  \\ & \qquad + 2  \mathbb E\left[\Big\| \frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]} \nabla F_i(y^i_{k-1})\Big\|^2 \bigg | C^t, y_0 \right]  
\end{align*}
Remark that in the inequality above, we cannot avoid the factor 2. This proves the second inequality.

% \begin{align*}
%     \mathbb{E}||\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\tilde{H}_i^k(y_i^{k-1})||^2 &= \mathbb{E}\big[||A||^2\big]\\
%     & \leq ||\mathbb{E}[A] ||^2 + \displaystyle\frac{\Sigma_g^2(C) + \varsigma^2/s\r}{KlM} && \text{(lemma \ref{lemma_mean_variance}-1 on $A$)} \\
%     &= \mathbb{E}||\displaystyle\frac{1}{KlM}\sum_{i \in C^t}\sum_{k \in [K]}\nabla F_i(y_i^{k-1}) ||^2 + \frac{\varsigma^2}{KlsM\r} + \frac{\Sigma_g^2(C)}{KlM}. 
% \end{align*}

\textbf{Third inequality.} We recall that for any $i \in C^t$,  $c_i=\frac{1}{K}\sum_{k=1}^K\tilde{H}_i^k(y_i^{k-1})$. Thus $\frac{1}{lM}\sum_{i \in C^t}c_i = A$ and we can directly use the results from the second and third inequalities. 
% We here define $B=\frac{1}{S}\sum_{i \in C^t}c_i$ conditionally to $\mathcal{Y}(C^t)$. From the definition of $c_i$, we remark that: $\mathbb{E}||c_i - \mathbb{E}[c_i]||^2 \leq (\varsigma^2/s\r + \Sigma^2_g(C))/K$. We then use the same steps as above and apply Lemma~\ref{lemma_mean_variance}-1 on B to obtain the inequality.\\

\textbf{Fourth inequality.} We recall that $c=\frac{1}{M}\sum_{i=1}^M c_i$ (even if local control variates are not updated). Therefore,
\begin{center}
    $\mathbb{E}[c]=\displaystyle\frac{1}{M}\sum_{i=1}^M \mathbb{E}[c_i]$ and $ \mathbb{E}|| c- \mathbb{E}[c]||^2\leq \displaystyle\frac{\varsigma^2/s\r + \Sigma^2_g(C)}{KM}\leq \frac{\varsigma^2}{KlsM\r} + \frac{\Sigma_g^2(C)}{KlM}$.
\end{center}

It finally comes that:
\begin{align*}
    \mathbb{E}||c||^2 &\leq || \displaystyle\frac{1}{M}\sum_{i=1}^M \mathbb{E}[c_i]||^2 + \frac{\varsigma^2}{KlsM\r} + \frac{\Sigma_g^2(C)}{KlM} && \text{(lemma \ref{lemma_mean_variance}-1 on $c$)}\\
    & \leq \displaystyle\frac{1}{M}\sum_{i=1}^M || \mathbb{E}[c_i]||^2 + \frac{\varsigma^2}{KlsM\r} + \frac{\Sigma_g^2(C)}{KlM} && \text{(Jensen inequality)}
\end{align*}
\end{proof}

\subsection{Theorem of convergence for \texttt{DP-SCAFFOLD-warm}}
\label{subsec_utility_dp_scaffold}

\begin{theorem}[Utility rates for \texttt{DP-SCAFFOLD-warm}, $\sigma_g$ chosen arbitrarily]\label{theorem_utility_scaffold}Let $\sigma_g, C>0$, $x^0 \in \mathbb{R}^d$. Suppose we run \texttt{DP-SCAFFOLD-warm}$(T,K,l,s,\sigma_g,C)$ with initial local controls such that $c_i^0=\frac{1}{K}\sum_{k=1}^K\tilde{H}_i^k(x^0)$ for any $i \in [M]$. Under Assumptions~\ref{ass:smooth_f_i} and \ref{ass:stoch_grad}, we  consider the sequence of iterates $(x^t)_{t\geq0}$ of the algorithm, starting from~$x^0$. 
\begin{enumerate}[topsep=0pt]
    \item If $F_i$ are \textbf{$\mu$-strongly convex} ($\mu>0$), $\eta_g=\sqrt{lM}$,
    $\eta_l = \min\big(\frac{l^{\frac{2}{3}}}{24\beta K\eta_g},\frac{l}{54\mu K \eta_g}\big)$,    and $T \geq \max (\frac{108}{l},\frac{48 \beta}{\mu l^{\frac{2}{3}}} )$,
    then, there exist weights $\{w_t\}_{t \in [T]}$ such that the averaged output of \texttt{DP-SCAFFOLD-warm}$(T,K,l,s,\sigma_g,C)$, defined by $\overline{x}^T=\sum_{t \in [T]} w_t x^t$, has expected excess of loss such that:
    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle\frac{\varsigma^2/s\r + \Sigma^2_g(C)}{\mu T K lM} + \mu D_0^2\exp(-\min\big(\frac{l}{108}, \frac{\mu l^{\frac{2}{3}}}{48 \beta}\big)T)\bigg)$,
    \end{center}
    \item If $F_i$ are \textbf{convex}, $\eta_g=\sqrt{lM}$, $\eta_l= \frac{l^{\frac{2}{3}}}{24\beta K\eta_g}$ and $T \geq 1$,then, there exist weights $\{w_t\}_{t \in [T]}$ such that the averaged output of \texttt{DP-SCAFFOLD-warm}$(T,K,l,s,\sigma_g,C)$, defined by $\overline{x}^T=\sum_{t \in [T]} w_t x^t$, has expected excess of loss such that:
    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle\frac{\varsigma/\sqrt{s\r} + \Sigma_g(C)}{\sqrt{TKlM}}D_0 + \frac{\beta}{l^{\frac{2}{3}}T}D_0^2 \bigg)$,
    \end{center}
    \item If $F_i$ are \textbf{non-convex}, $\eta_g=\sqrt{lM}$, $\eta_l = \frac{l^{\frac{2}{3}}}{24\beta K\eta_g}$ and $T \geq 1$, then there exist weights $\{w_t\}_{t \in [T]}$ such that the randomized  output of \texttt{DP-SCAFFOLD-warm}$(T,K,l,s,\sigma_g,C)$, defined by $\{\overline{x}^T= x^t \text{ with probability } w_t \text{ for all } t\}$, has expected squared gradient of the loss such that:
\begin{center}
    $\mathbb{E}||\nabla F(\overline{x}^T)||^2 \leq \mathcal{O}\bigg(\displaystyle\frac{\varsigma/\sqrt{s\r} + \Sigma_g(C)}{\sqrt{TKlM}}\sqrt{F_0} +\frac{\beta}{l^{\frac{2}{3}} T}F_0\bigg)$,
\end{center}
% \end{itemize}
\end{enumerate}
where $D_0=||x^0 - x^*||$ and $F_0:=F(x^0) - F^*$.
\end{theorem}

We recover the result of Theorem~\ref{utility_result} for \texttt{DP-SCAFFOLD-warm} where $F_i$ are convex by setting $\sigma_g=\sigma_g^*$ where $\sigma_g^*:=s\sqrt{lTK\log(2Tl/\delta)\log(2/\delta)}/\epsilon\sqrt{M}$, which gives $\Sigma_g(C)=2Cd\sqrt{2lTK\log(2Tl/\delta)\log(2/\delta)}/\epsilon\r\sqrt{M}$ (with numerical constants omitted for the asymptotic bound).

\subsection{Proof of Theorem~\ref{theorem_utility_scaffold} (Convex case)}
\label{subsec_utility_dp_scaffold_convex}

In this section, we detail the proof of convergence of \texttt{DP-SCAFFOLD-warm} with convex local loss functions. This proof is adapted from the proof given by \cite{fl_scaffold} without DP noise. We use below the notations from Section~\ref{algo_description}.\\



\paragraph{Summary of the main steps.}

Let $t \in [T]$ be an arbitrary communication round of the algorithm. We detail below the updates that occur at this round.
\begin{itemize}
    \item Let $i \in C^t$. Starting from $y_{i}^0=x^{t-1}$, the random variable $y_i$ is updated at local step $k\in [K]$ such that $y_{i}^k:=y_{i}^{k-1} - \eta_l v_{i,k}^t$ where $v_{i,k}^t=\tilde{H}_i^k(y_{i}^{k-1}) - c_i^{t-1} + c^{t-1}$.
    \item Then we define the local control variate $\tilde{c}_i^t$ for this user by:
    \begin{align*}
        \tilde{c}_i^t:=c^{t-1} - c_i^{t-1} + \displaystyle\frac{1}{K \eta_l}(x^{t-1}- y_i^K)=\frac{1}{K}\sum_{k=1}^K\tilde{H}_i(y_i^{k-1}).
    \end{align*}
    \item For any $i \in [M]$, we update the control variate $c_i^t$ such that:
    \begin{itemize}
        \item $c_i^t:=\tilde{c}_i^t$ if $i \in C^t$,
        \item $c_i^t:=c_i^{t-1}$ otherwise.
    \end{itemize}
    \item Finally, the global update is computed as:
    \begin{center}
        $x^t=x^{t-1}+\displaystyle\frac{\eta_g}{lM}\sum_{i \in C^t}(y_i^K - x^{t-1})$
        and $c^t=\displaystyle\frac{1}{M}\big(\sum_{i \in C^t}c_i^t + \sum_{i \notin C^t}c_i^{t-1}\big)$.
    \end{center}
\end{itemize}

To keep track of the lag in the update of $c_i^t$, we introduce $\alpha_{i,k-1}^t$ defined for any $i \in[M]$, any $t \in [T]$ and any $k \in [K]$ by:
\begin{align*}
    \alpha_{i,k-1}^t =\left\{
    \begin{array}{ll}
        y_i^{k-1} & \text{ if } i \in C^t \\
        \alpha_{i,k-1}^{t-1}& \text{ otherwise}
    \end{array}
        \right.
\end{align*}
with $\alpha_{i,k-1}^0=x^0$.

We hence have the following property for any $i \in [M]$ and any $t\in [T]$: $c_i^t= \frac{1}{K}\sum_{k=1}^K\tilde{H}_i^k(\alpha_{i,k-1}^t)$.

\textbf{Additional definitions.}
\begin{itemize}[noitemsep,topsep=0pt]
    \item Model gap: $\Delta x^t:=x^t -x^{t-1}$,
    \item Global step-size: $\tilde{\eta}:=K\eta_l \eta_g$ which gives $\Delta x^t = -\displaystyle\frac{\tilde{\eta}}{KlM}\sum_{k\in[K], i \in C^t} \tilde{H}_i^k (y_i^{k-1}) + c^{t-1} - c_i^{t-1}$,
    \item User-drift: $\mathcal{E}_t:=\displaystyle\frac{1}{KM}\sum_{k=1}^K \sum_{i=1}^M \mathbb{E} || y_i^k - x^{t-1}||^2$, 
    \item Control lag: $\mathcal{F}_t:=\displaystyle\frac{1}{KM}\sum_{k=1}^K \sum_{i=1}^M \mathbb{E} || \alpha_{i,k-1}^t - x^{t}||^2$ with $\mathcal{F}_0=0$.
\end{itemize}


\textbf{Originality of the proof.} The proof substantially differs form the proof by \citet{fl_scaffold} in the convex case. Indeed,  \citet{fl_scaffold} control a combination of the quadratic distance to the optimum and a control of the deviation between the controls   and the gradients at the optimal point $\|c_i^t -\nabla F_i(x^*)\|.$ Leveraging such a quantity in our proof would  result in a worse upper bound on the utility than the one we get, as either the noise added to ensure DP (if $c_i^0$ is defined w.r.t. a noised gradient) or the heterogeneity (if $c_i^0=0$)  would also appear in the initial
condition $\|c_i^t -\nabla F_i(w^*)\|.$
On the other hand, in our approach, we combine the  quadratic distance to the optimum to a control of the lag and user-drift. In some sense this resembles some aspects of the proof in the non-convex regime in \citep{fl_scaffold}, in which the excess risk ($F(x_t) - F^*$) is combined with the lag. However, our result (in the convex case), strongly leverages the convexity of the function in the proof.

\paragraph{Details of the proof.}

The idea of the proof is to find a contraction inequality involving $||x^t - x^*||^2$, $\mathbb{E}[F(x^{t-1})] - F(x^*)$, $\mathcal{F}_t$ and $\varsigma/\sqrt{s\r} + \Sigma_g(C)$. To do so, we will first bound the variance of the server's update. Then we will see how the control lag evolves through the communication rounds. We will also bound the user drift. To make the proof more readable, the index $t$ may be omitted on random variables when the only communication round that is considered is the $t$-th one.\\

\begin{lemma}[\textbf{Variance of the server's update}]
\leavevmode
$\forall \tilde{\eta} \in [0, 1/\beta]$

\begin{itemize}
    \item $\mathbb{E}||\mathbb{E}_{t-1}(x^t) - x^{t-1}||^2 \leq 2 \tilde{\eta}^2\beta^2\mathcal{E}_t + 4 \beta \tilde{\eta}^2 \mathbb{E}\big(F(x^{t-1}) -F(x^*)\big)$,
    \item $\mathbb{E}||x^t - x^{t-1}||^2 \leq 4 \tilde{\eta}^2\beta^2 \mathcal{E}_t + 8 \beta^2 \tilde{\eta}^2 \mathcal{F}_{t-1} + 8 \beta \tilde{\eta}^2 \mathbb{E}\big(F(x^{t-1}) -F(x^*)\big) + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C))$.
\end{itemize}
\end{lemma}

\begin{proof} We consider the model gap $\Delta x^t = x^t-x^{t-1}$
\begin{align*}
    \mathbb{E}||\Delta x^t||^2=\tilde{\eta}^2 \mathbb{E}\Big\|\underbrace{\bigg(\frac{1}{KlM}\sum_{k\in [K], i\in C^t} \tilde{H}_i(y_i^{k-1})\bigg)}_{A_1} + \underbrace{c^{t-1}}_{A_2} -\underbrace{\frac{1}{lM}\sum_{i \in C^t} c_i^{t-1}}_{A_3} \Big\|^2
\end{align*}
% \aymeric{dans la ligne au dessus, on souffre un peu de ne pas avoir les indices t...:) }
% \maxence{il manque des espérances pour donner les quantités d'intérêt}

We combine Lemma~\ref{lemma_mean_variance}-1 on $A_1, A_2, A_3$ with Corollary~\ref{corollary_noise} which controls their individual variance by $\frac{\varsigma^2/s\r + \Sigma_g^2(C)}{KlM}$. It leads to:
\begin{align*}
    \mathbb{E}||\Delta x^t||^2 & = \tilde{\eta}^2\mathbb{E}\left[  \mathbb E \left[ \bigg\| \bigg(\frac{1}{KlM}\sum_{k\in [K], i\in C^t} \tilde{H}_i(y_i^{k-1})\bigg)+ c^{t-1}- \frac{1}{lM}\sum_{i \in C^t} c_i^{t-1} \bigg\|^2 \bigg| C^t \right]  \right]\\ 
    % & = 4 \tilde{\eta}^2\mathbb{E}\left[  \mathbb E \left[ \bigg\| \bigg(\frac{1}{KlM}\sum_{k\in [K], i\in C^t} \tilde{H}_i(y_i^{k-1}) - \nabla F_i(x) \bigg)+ c^{t-1} -\nabla F(x)  - \sum_{i \in C^t} c_i^{t-1} - \nabla F_i(x) \bigg\|^2 \bigg| C^t \right]  \right]\\ 
    % & \\
    & \le \tilde{\eta}^2\mathbb{E}\left[\Big\|\frac{1}{KlM}\sum_{k\in [K], i\in C^t} \nabla F_i(y_i^{k-1}) + \mathbb{E}(c) - \mathbb{E}(c_i)\Big\|^2\right] + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C))\\
    & \leq \tilde{\eta}^2 \mathbb{E}\left[\frac{1}{KlM}\sum_{k\in [K], i\in C^t} \Big\| \nabla F_i(y_i^{k-1}) + \mathbb{E}(c) - \mathbb{E}(c_i)\Big\|^2 \right] + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)) & \text{(convexity of $||.||^2$)}\\
    & = \tilde{\eta}^2 \frac{1}{KM}\sum_{k, i}\mathbb{E}\Big[ \Big\| \underbrace{\nabla F_i(y_i^{k-1}) + \mathbb{E}(c) - \mathbb{E}(c_i)}_{\substack{\nabla F_i(y_i^{k-1}) - \nabla F_i(x) \\ + \mathbb{E}(c) - \nabla F(x) \\ + \nabla F(x) \\ - \mathbb{E}(c_i) + \nabla F_i(x)}}\Big\|^2 \Big] + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)) & \text{(definition of $C^t$)}\\
    & \leq \frac{4 \tilde{\eta}^2}{KM}\sum_{k,i}\mathbb{E}\left[\Big\|\nabla F_i(y_i^{k-1}) - \nabla F_i(x)\Big\|^2\right] + \frac{8 \tilde{\eta}^2}{KM} \sum_{k,i}\mathbb{E}\left[\Big\|\nabla F_i(\alpha_{i, k-1}) - \nabla F_i(x)\Big\|^2\right] \\
    & + 4\tilde{\eta}^2 \mathbb{E}\Big\|\nabla F(x)\Big\|^2 + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)).
\end{align*}
The last inequality is obtained by definition of $c$ and $c_i$ and by relaxed triangle inequality. With Lemma~\ref{lemma_nesterov}, this leads to the second result. The first one can be obtained in the same way.
\end{proof}

\begin{lemma}[\textbf{Lag in the control variate}] 
\label{control_variable_lemma}
\leavevmode
$\forall \alpha \in [1/2, 1], \forall \tilde{\eta} \leq \frac{1}{24 \beta}l^{\alpha}$,
\begin{align*}
    \mathcal{F}_t \leq \left(1 -\frac{17}{36}l\right)\mathcal{F}_{t-1} + \frac{1}{24 \beta} l^{2 \alpha -1} \mathbb{E}\big(F(x^{t-1}) -F(x^*)\big) + \frac{97}{48}l^{2 \alpha -1}\mathcal{E}_t + \frac{l}{\beta^2}\frac{\varsigma^2/s\r + \Sigma_g^2(C)}{32 KlM}.
\end{align*}
\end{lemma}

\begin{proof}
We adapt the original proof made in the non-convex case \cite[Lemma 16]{fl_scaffold} and use Lemma~\ref{lemma_reg_h_tilde} and Lemma~\ref{lemma_nesterov}.  
\end{proof}

\begin{lemma}[\textbf{Bounding the user drift}]
\label{user_drift}
\leavevmode
$\forall \eta_g \geq 1, \forall \eta_l \leq 1/24\beta K \eta_g$,
\begin{align*}
    \frac{9}{2}\beta^2\tilde{\eta} \mathcal{E}_t \leq \frac{9}{2}\beta^3\tilde{\eta}^2 \mathcal{F}_{t-1} + \frac{9}{40}\frac{\tilde{\eta}\beta}{\eta_g^2} \mathbb{E}\big(F(x^{t-1}) -F(x^*)\big) + \frac{27}{40}\frac{\tilde{\eta}^2 \beta}{K \eta_g^2} \big(\varsigma^2/s\r + \Sigma_g^2(C)\big).
\end{align*}
\end{lemma}
\begin{proof}

We once again adapt the original proof made in the non-convex case \cite[Lemma 17]{fl_scaffold}, use Lemma~\ref{lemma_nesterov} and multiply on each side of the inequality by $\frac{9}{2}\beta^2\tilde{\eta}$.
\end{proof}


\begin{lemma}[\textbf{Progress made at each round}]
\leavevmode
\label{progress_round}
$\forall \eta_g \geq 1, \forall \eta_l \leq \min \big(\frac{1}{24 K \eta_g \beta}l^{2/3}, \frac{l}{54\mu K\eta_g}\big)$,
\begin{align*}
    \mathbb{E}||x^t - x^*||^2 + 27 \beta^2 \tilde{\eta}^2 \frac{1}{l}\mathcal{F}_t & \leq \left(1 - \frac{\mu \tilde{\eta}}{2}\right)\left[\mathbb{E}||x^{t-1} -x^*||^2 + 27 \beta^2 \tilde{\eta}^2 \frac{1}{l}\mathcal{F}_{t-1} \right]\\
    & - \frac{\tilde{\eta}}{2}\mathbb{E}\big(F(x^{t-1}) -F(x^*)\big) + \frac{10 \tilde{\eta}^2}{KlM}\left(1+\frac{S}{\eta_g^2}\right)(\sigma^2 +\Sigma^2).
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
    \mathbb{E}_{t-1}||x + \Delta x - x^*||^2 & = \mathbb{E}_{t-1}||x - x^*||^2 + \mathbb{E}_{t-1}||\Delta x||^2 - \frac{2 \tilde{\eta}}{KlM}\mathbb{E}_{t-1}\left[\sum_{k \in [K],i \in C^t}\langle \nabla F_i(y_i^{k-1}), x - x^* \rangle \right]\\
    & \leq \mathbb{E}_{t-1}||x - x^*||^2 + 4 \tilde{\eta}^2\beta^2 \mathcal{E}_t + 8 \beta^2 \tilde{\eta}^2 \mathcal{F}_{t-1} + 8 \beta \tilde{\eta}^2 \mathbb{E}\left(F(x^{t-1}) -F(x^*)\right)\\
    & + \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)) + \underbrace{\frac{2 \tilde{\eta}}{KlM}\mathbb{E}_{t-1}\left[\sum_{k \in [K],i \in C^t}\langle \nabla F_i(y_i^{k-1}), x^* -x \rangle \right]}_{\mathcal{A}},
\end{align*}

where
\begin{align*}
    \mathbb{E}[\mathcal{A}] & \leq \frac{2 \tilde{\eta}}{KlM}\mathbb{E}\left(\sum_{k\in [K], i\in C^t} F_i(x^*) -F_i(x) + \beta ||y_i^{k-1} -x||^2 - \frac{\mu}{4}||x - x^*||^2\right) & \text{(convexity and $\beta$-smoothness)}\\
    & = - 2 \tilde{\eta}\left(\mathbb{E}(F(x)) - F(x^*) + \frac{\mu}{4}\mathbb{E}||x-x^*||\right) + 2 \beta \tilde{\eta}\mathcal{E}_t.
\end{align*}

Hence: 
\begin{align*}
    \mathbb{E}||x + \Delta x - x^*||^2 & \leq \mathbb{E}||x - x^*||^2 - 2 \tilde{\eta}\left(\mathbb{E}(F(x)) - F(x^*) + \frac{\mu}{4}\mathbb{E}||x-x^*||^2\right) + 2 \beta \tilde{\eta}\mathcal{E}_t\\
    & + 4 \tilde{\eta}^2\beta^2 \mathcal{E}_t + 8 \beta^2 \tilde{\eta}^2 \mathcal{F}_{t-1} + 8 \beta \tilde{\eta}^2 \mathbb{E}\left(F(x^{t-1}) -F(x^*)\right)+ \frac{9\tilde{\eta}^2}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)).
\end{align*}

By combining all terms and multiplying by $\beta$ on each side of the inequality, it comes:
\begin{align}
    \label{first_inequ}
    \beta \mathbb{E}||x + \Delta x - x^*||^2 & \leq
    \left(1 - \frac{\mu \tilde{\eta}}{2}\right)\beta \mathbb{E}||x-x^*||^2 + (8 \beta^2\tilde{\eta}^2 - 2\tilde{\eta} \beta) \left(\mathbb{E}(f(x^{t-1})) - F(x^*)\right)\\
    & + \frac{9\tilde{\eta}^2\beta}{KlM}(\varsigma^2/s\r + \Sigma_g^2(C)) + (2 \beta^2\tilde{\eta} + 4 \beta^3\tilde{\eta}^2)\mathcal{E}_t + 8 \beta^3 \tilde{\eta}^2 \mathcal{F}_{t-1} \nonumber.
\end{align}

We now consider $\alpha \in [1/2, 1]$, $\eta_l \leq \frac{1}{24 K \beta \eta_g} l^\alpha$ and $\eta_g \geq 1$. We use the result of Lemma~\ref{control_variable_lemma} where each side is multiplied by $27\beta^3\tilde{\eta}^2\frac{1}{l}$ to obtain:

\begin{align}
\label{second_inequ}
    27\beta^3\tilde{\eta}^2\frac{1}{l}\mathcal{F}_t & \leq \big(1-\frac{\mu \tilde{\eta}}{2}\big)27\beta^3\tilde{\eta}^2\frac{1}{l}\mathcal{F}_{t-1} + 27 \big(\frac{\mu \tilde{\eta}}{2l}- \frac{17}{36}\big)\beta^3\tilde{\eta}^2\mathcal{F}_{t-1}\\
    & + \frac{9}{8}l^{2\alpha -2}\beta^2 \tilde{\eta}^2 \big(\mathbb{E}(f(x^{t-1})) - F(x^*)\big) + \frac{873}{16}l^{2\alpha -2}\beta^3\tilde{\eta}^2\mathcal{E}_t \nonumber\\
    & +\frac{27}{32}\beta \tilde{\eta}^2 \frac{\varsigma^2/s\r + \Sigma_g^2(C)}{KlM} \nonumber.
\end{align}

Since we have $\eta_l \leq \frac{1}{24 K \beta \eta_g}$, we recall the result from Lemma~\ref{user_drift}: 

\begin{align}
\label{third_inequ}
    \frac{9}{2}\beta^2\tilde{\eta} \mathcal{E}_t \leq \frac{9}{2}\beta^3\tilde{\eta}^2 \mathcal{F}_{t-1} + \frac{9}{40}\frac{\tilde{\eta}\beta}{\eta_g^2} \mathbb{E}\big(F(x^{t-1}) -F(x^*)\big) + \frac{27}{40}\frac{\tilde{\eta}^2 \beta}{K \eta_g^2} \big(\varsigma^2/s\r + \Sigma_g^2(C)\big).
\end{align}

By summing inequalities (\ref{first_inequ}), (\ref{second_inequ}), (\ref{third_inequ}), we obtain:
\begin{align}
    \beta \mathbb{E}||x^t - x^*||^2 + 27\beta^3\tilde{\eta}^2\frac{1}{l}\mathcal{F}_t & \leq \big(1-\frac{\mu \tilde{\eta}}{2}\big)\big(\beta \mathbb{E}||x - x^*||^2 + 27\beta^3\tilde{\eta}^2\frac{1}{l}\mathcal{F}_{t-1}\big) \nonumber\\
    & + \big( \frac{9}{8}l^{2\alpha -2}\beta^2 \tilde{\eta}^2 + \frac{9}{40}\frac{\tilde{\eta}\beta}{\eta_g^2} +  8 \beta^2\tilde{\eta}^2 - 2\tilde{\eta} \beta\big)\big(\mathbb{E}(F(x)) - F(x^*)\big) \label{first_part}\\
    & + \big(\frac{315}{32} +\frac{27}{40}\frac{lM}{\eta_g^2}\big)\frac{\tilde{\eta}^2 \beta}{K lM} \big(\varsigma^2/s\r + \Sigma_g^2(C)\big) \label{second_part}\\
    & + \big(-\frac{5}{2}\beta \tilde{\eta} + 4 \beta^2\tilde{\eta}^2 + \frac{873}{16}l^{2\alpha -2}\beta^2\tilde{\eta}^2\big)\beta \mathcal{E}_t \label{third_part}\\
    & +\big(27\big(\frac{\mu\tilde{\eta}}{2l}-\frac{17}{36}\big)\beta^2\tilde{\eta}^2 + \frac{25}{2}\beta^2\tilde{\eta}^2\big)\beta\mathcal{F}_{t-1} \label{fourth_part}.
\end{align}


We now consider $\eta_l \leq l/54\mu K \eta_g$. Then $\tilde{\eta}\leq l/54\mu$ and we recall that $\beta \tilde{\eta} \leq 1/24$. We fix $\alpha=2/3$ (then $2 - 2\alpha=\alpha)$.\\

In this part, we aim at simplifying the terms on the right side of the last inequality.\\

\textbf{Simplifying (\ref{first_part}):}
\begin{align*}
    \frac{9}{8}l^{2\alpha -2}\beta^2 \tilde{\eta}^2 + \frac{9}{40}\frac{\tilde{\eta}\beta}{\eta_g^2} +  8 \beta^2\tilde{\eta}^2 - 2\tilde{\eta} \beta & \leq \big(\frac{9}{8\times 24} +\frac{9}{40}+ \frac{8}{24} -2\big)\beta\tilde{\eta}\\
    & = -\underbrace{\frac{1339}{960}}_{\sim 1.39}\beta\tilde{\eta} \leq -\frac{\beta\tilde{\eta}}{2}.
\end{align*}

\textbf{Simplifying (\ref{second_part}):}
\begin{align*}
    \frac{315}{32} +\frac{27}{40}\frac{lM}{\eta_g^2} \leq 10 \big(1 +\frac{lM}{\eta_g^2}\big).
\end{align*}

\textbf{Simplifying (\ref{third_part}):}\\

Since $l^{2\alpha -2}\beta\tilde{\eta}= \beta\tilde{\eta}\big(\frac{1}{l}\big)^{2/3}\leq 1/24$, 
\begin{align*}
    -\frac{5}{2}\beta \tilde{\eta} + 4 \beta^2\tilde{\eta}^2 + \frac{873}{16}l^{2\alpha -2}\beta^2\tilde{\eta}^2 & \leq \big(-\frac{5}{2} + \frac{4}{24} + \frac{873}{16}\frac{1}{24}\big)\beta\tilde{\eta}\\
    & = -\frac{23}{384}\beta\tilde{\eta} \leq 0.
\end{align*}

\textbf{Simplifying (\ref{fourth_part}):}\\

Since $\frac{\mu \tilde{\eta}}{2l}\leq 1/108$,
\begin{align*}
    27\big(\frac{\mu\tilde{\eta}}{2l}-\frac{17}{36}\big)\beta^2\tilde{\eta}^2 + \frac{25}{2}\beta^2\tilde{\eta}^2 \leq \big(27(\frac{1}{108}-\frac{17}{36}) + \frac{25}{2}\big)\beta^2\tilde{\eta}^2 =0.
\end{align*}

We then obtain the final result by dividing by $\beta$ on each side of the inequality.
\end{proof}

\begin{lemma}[\textbf{Convergence of \texttt{DP-SCAFFOLD-warm}  with convex loss functions}]\label{lemma_utility_with_contraction} There exist weights $\{w_t\}$ such that $\overline{x}^T=\sum_{t \in [T]} w_t x^t$ and:
    \item If $f_i$ are \textbf{$\mu$-strongly convex} ($\mu>0$), $\eta_g\geq 1$,
    $\eta_l \leq \min\big(\frac{l^{\frac{2}{3}}}{24\beta K\eta_g},\frac{l}{54\mu K \eta_g}\big)$,
    and $T \geq \max (\frac{108}{l},\frac{48 \beta}{\mu l^{\frac{2}{3}}} )$,

    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle\frac{\varsigma^2/s\r + \Sigma_g^2(C)}{\mu T KlM}\big(1 + \frac{lM}{\eta_g^2}\big) + \mu D_0^2\exp(-\min\big(\frac{l}{108}, \frac{\mu l^{\frac{2}{3}}}{48 \beta}\big)T)\bigg)$,
    \end{center}
    
    \item If $f_i$ are \textbf{convex}, $\eta_g\geq 1$, $\eta_l\leq \frac{l^{\frac{2}{3}}}{24\beta K\eta_g}$ and $T \geq 1$,
    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle D_0\frac{\varsigma/\sqrt{s\r} + \Sigma_g(C)}{\sqrt{TKlM}}\sqrt{1 + \frac{lM}{\eta_g^2}} + \frac{\beta}{T}D_0^2(\frac{1}{l})^{\frac{2}{3}} \bigg)$,
    \end{center}

where $D_0:=||x^0 - x^*||$.
\end{lemma}
\begin{proof}
The result of Lemma~\ref{lemma_utility_with_contraction} is obtained by combining the contraction inequality from Lemma~\ref{progress_round} and the results from technical contraction results \cite[Lemmas 1 and 2]{fl_scaffold}.
\end{proof}

We then obtain the result of Theorem~\ref{theorem_utility_scaffold} by setting $\eta_g:=\sqrt{lM} \geq 1$ and $\eta_l$ as low as possible.

\subsection{Proof of Theorem~\ref{theorem_utility_scaffold} (Non-Convex case)}
\label{subsec_utility_dp_scaffold_non_convex}

To state this result, we adapt the original proof in the case with a larger variance for DP-noised stochastic gradients (see Lemma~\ref{lemma_reg_h_tilde}), which gives the following result.

\begin{lemma}[\textbf{Convergence of \texttt{DP-SCAFFOLD-warm}  with non-convex loss functions}] There exist weights $\{w_t\}$ such that $\overline{x}^T=\sum_{t \in [T]} w_t x^t$ and:
    \item If $f_i$ are \textbf{non-convex}, $\eta_g\geq 1$, $\eta_l\leq \frac{l^{\frac{2}{3}}}{24\beta K\eta_g}$ and $T \geq 1$,
    \begin{center}
        $\mathbb{E}||\nabla F(\overline{x}^T)||^2 \leq \mathcal{O}\bigg(\displaystyle\frac{(\varsigma/\sqrt{s\r} + \Sigma_g(C))\sqrt{F_0} }{\sqrt{TKlM}}\sqrt{1 + \frac{lM}{\eta_g^2}} +\frac{\beta}{T}F_0 (\frac{1}{l})^{\frac{2}{3}}\bigg)$,
    \end{center}
where $F_0:=F(x^0) - F(x^*)$.
\end{lemma}

We obtain the result of Theorem~\ref{theorem_utility_scaffold} by setting $\eta_g:=\sqrt{lM} \geq 1$ and $\eta_l$ as low as possible.

\subsection{Theorem of convergence for \texttt{DP-FedAvg}}
\label{subsec_utility_dp_fedavg}

\begin{theorem}[Utility rates of \texttt{DP-FedAvg}$(T,K,l,s,\sigma_g,C)$, $\sigma_g$ chosen arbitrarily]\label{theorem_utility_fedavg}Let $\sigma_g, C>0$, $x^0 \in \mathbb{R}^d$. Suppose we run \texttt{DP-FedAvg}$(T,K,l,s,\sigma_g,C)$ (see Algorithm~\ref{algo_dp_fedavg}). Under Assumptions~\ref{ass:smooth_f_i} and \ref{ass:stoch_grad}, we  consider the sequence of iterates $(x^t)_{t\geq0}$ of the algorithm, starting from $x^0$. 

\begin{enumerate}
    \item If $F_i$ are \textbf{$\mu$-strongly convex} ($\mu>0$), $\eta_g=\sqrt{lM}$, $\eta_l= \frac{1}{8(1+B^2)\beta K\eta_g}$ and $T\geq \frac{8(1+b^2)\beta}{\mu}$, then  there exist weights $\{w_t\}_{t \in [T]}$ such that the averaged output of \texttt{DP-FedAvg}$(T,K,l,s,\sigma_g,C)$, defined by $\overline{x}^T=\sum_{t \in [T]} w_t x^t$, has expected excess of loss such that:
    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle \frac{\varsigma^2/s\r + \Sigma_g^2(C)}{\mu TKlM} + (1-l) \frac{G^2}{\mu T lM} + \frac{\beta G^2}{\mu^2 T^2} + \mu D_0^2 \exp(-\frac{\mu}{16(1+B^2)\beta}T)\bigg)$,
    \end{center}
    
    \item If $F_i$ are \textbf{convex}, $\eta_g=\sqrt{lM}$, $\eta_l= \frac{1}{8(1+B^2)\beta K\eta_g}$ and $T \geq 1$,  then  there exist weights $\{w_t\}_{t \in [T]}$ such that the averaged output of \texttt{DP-FedAvg}$(T,K,l,s,\sigma_g,C)$, defined by $\overline{x}^T=\sum_{t \in [T]} w_t x^t$, has expected excess of loss such that:
    \begin{center}
        $\mathbb{E}[F(\overline{x}^T)] -F(x^*) \leq \mathcal{O}\bigg(\displaystyle D_0\frac{\varsigma/\sqrt{s\r} + \Sigma_g(C)}{\sqrt{TKlM}} + \frac{GD_0\sqrt{1-l}}{\sqrt{T lM}} + \frac{D_0^{4/3}\beta^{1/3}G^{2/3}}{T^{2/3}} + \frac{B^2\beta D_0^2}{T} \bigg)$,
    \end{center}
    
    \item If $F_i$ are \textbf{non-convex}, $\eta_g=\sqrt{lM}$, $\eta_l= \frac{1}{8(1+B^2)\beta K\eta_g}$ and $T \geq 1$,  then there exist weights $\{w_t\}_{t \in [T]}$ such that the randomized  output of \texttt{DP-SCAFFOLD-warm}$(T,K,l,s,\sigma_g,C)$, defined by $\{\overline{x}^T= x^t$ with probability $w_t$ for all $t\}$, has expected squared gradient of the loss such that:
    \begin{center}
        $\mathbb{E}||\nabla F(\overline{x}^T)||^2 \leq \mathcal{O}\bigg(\displaystyle \frac{\beta (\varsigma/\sqrt{s\r} + \Sigma_g(C))\sqrt{F}}{\sqrt{TKlM}} + \frac{\beta G \sqrt{F(1-l)}}{\sqrt{TlM}} + \frac{F^{2/3}\beta^{1/3}G^{2/3}}{T^{2/3}} + \frac{B^2 \beta F}{T}\bigg)$,
    \end{center}
\end{enumerate}
where $D_0:=||x^0 - x^*||$ and $F:=f(x^0) - f^*$.
\end{theorem}


























\begin{proof}
To state the result of Theorem~\ref{theorem_utility_fedavg}, we combine the original result \cite[Theorem V]{fl_scaffold} provided for any type of loss functions with the result of Lemma~\ref{lemma_reg_h_tilde}.
\end{proof}

% \newpage
\section{Additional Experimental Details and Results}
\label{app:exp_all}

In this section, we give additional details on our experimental setup (Section~\ref{app:setting_algo}) and simulated data generation process (Section~\ref{app:data_gen}), and provide additional results (Section~\ref{appendix_experiment}).

\subsection{Algorithms Setup}
\label{app:setting_algo}

\paragraph{Hyperparameter tuning.} 

We tuned the step size hyperparameter $\eta_0$ for each dataset, each algorithm and each noise version (with or without DP) over a grid of 10 values with the lowest level of heterogeneity (5-fold cross validation conducted on the training set). We kept the same $\eta_0$ for the experiments with higher heterogeneity.

\paragraph{Clipping heuristic.} 

Setting a good clipping threshold $C$ while preserving accuracy can be difficult  \citep{dp_fedavg_user_level}. Indeed, if $C$ is too small, the clipped gradients may become biased, thereby affecting the convergence rate. On the other hand, if $C$ is too large, we have to add more noise to stochastic gradients to ensure differential privacy (since the variance of the Gaussian noise is proportional to $C^2$). In practice, we follow the strategy proposed by \citet{dp_deep_l}, which consists in setting $C$ as the median of the norms of the unclipped gradients over each stage of local training. Throughout the iterations, $C$ will then decrease. However, we are aware that locally setting $C$ may leak information to the server about the magnitude of stochastic gradients. We here consider this leak as minor and neglect its impact on privacy guarantees. Adaptive clipping \citep{dp_adaptive_clipping} could be used to mitigate these concerns.


\subsection{Simulated Data Generation}
\label{app:data_gen}

% \paragraph{Details on simulated data.}

Each ground-truth model for a user $i$ consists of weights $W_i \in \mathbb{R}^{d'\times 10}$ and bias $b_i \in \mathbb{R}^{10}$, which are sampled from the following distributions: $ W_i | u_i \sim \mathcal{N}_{d' \times 10}(u_i,\text{Id})$ and $b_i |u_i' \sim \mathcal{N}_{10}(u_i', \text{Id})$ where $u_i \sim \mathcal{N}_{d' \times 10}(0, \alpha \text{Id})$ and $u_i' \sim \mathcal{N}_{10}(0, \alpha \text{Id})$. The data matrix $X_i$ of user $i$ is sampled according to $X_i |v_i \sim \mathcal{N}_{d'}(v_i, \Sigma)$ where $\Sigma$ is the covariance matrix defined by its diagonal $\Sigma_{j,j}=j^{-1.2}$ and $v_i |B_i \sim \mathcal{N}_{d'}(B_i,\text{Id})$ where $B_i \sim \mathcal{N}_{d'}(0,\beta\text{Id})$.
The label of each data point is obtained by independently changing the label given by the ground-truth model with probability $0.05$.

% \paragraph{Details on real-world data}
% \maxence{Rien à rajouter par rapport à ce qui est dans le main}

\subsection{Experiments}
\label{appendix_experiment}

In this section, we provide more results on the experiments described in Section~\ref{sec:experiments}, and also present additional experiments.

\paragraph{Metrics.} 

To measure the convergence and performance of the algorithms at any communication round $t\in [T]$, we consider the following metrics:
\begin{itemize}
    \item \textit{Accuracy(t)}: the average test accuracy of the model over all users,
    \item \textit{Train Loss(t)}$=\log_{10} (F(x^t)-F^*)$: the log-gap between the objective function evaluated at parameter $x^t$ and its minimum,
    \item \textit{Train Gradient Dissimilarity(t)}$=\frac{1}{M}\sum_{i=1}^M ||\nabla F_i(x^t)||^2 - ||\nabla F(x^t)||^2$, which measures how the local gradients differ from the global gradient (i.e., the average across users) when evaluated at $x^t$, and hence quantifies the \textit{user-drift} over the rounds of communication. Remark that, without any kind of heterogeneity, this variable would converge to 0.
\end{itemize}

\paragraph{Experiments with $TK$ fixed.}

In Section~\ref{sec:experiments} of the main text, we conducted experiments on both FEMNIST and simulated data with a total number of iterations that is \textit{constant} %, in order to simulate real-world material constraints
($TK=4.10^4$ for FEMNIST data and $TK=8.10^4$ for simulated data). As observed in previous work \citep{fl_scaffold}, these experiments recover the superiority of \texttt{SCAFFOLD} over \texttt{FedAvg} and \texttt{FedSGD} under heterogeneous data, but most importantly they show that this hierarchy is preserved in our DP-FL framework with privacy constraints: this is especially clear with growing heterogeneity and with growing number $K$ of local updates. Besides this, the results provided for logistic regression in the high-privacy regime ($\epsilon=1.5$) numerically demonstrate that \textbf{\texttt{DP-SCAFFOLD-warm} actually outperforms (non-private) \texttt{FedAvg}} (see Fig.~\ref{logistic_20_epochs_heterogene}), despite the local injection of Gaussian noise! Therefore, our results are quite promising with respect to obtaining efficient DP-FL algorithms under heterogeneous data.

We provide below some additional results which complement those provided in Section~\ref{sec:experiments}. 
\begin{itemize}
    \item \textbf{Simulated data.} We plot in Fig.~\ref{logistic_10_20_epochs_accuracy} the evolution of the accuracy over the rounds, which is consistent with the evolution of the train loss in Fig.~\ref{logistic_20_epochs_heterogene}. While the variance of the accuracy for \texttt{DP-FedAvg} grows with the heterogeneity, the results of \texttt{DP-SCAFFOLD-warm} are not affected. We can observe an average difference of $10\%$ in the accuracy for these two algorithms over the various heterogeneity settings. We provide in Fig.~\ref{logistic_10_20_epochs_diss} the evolution of the gradient dissimilarity for the same settings as in Fig.~\ref{logistic_20_epochs_heterogene} and Fig.~\ref{logistic_10_20_epochs_accuracy}, which once again shows a better convergence of \texttt{DP-SCAFFOLD-warm} compared to \texttt{DP-FedAvg} for the same privacy level. We also provide the evolution of the train loss when varying a single heterogeneity parameter: either $\alpha$ (which controls \textit{model} heterogeneity across users) in Fig.~\ref{logistic_10_20_epochs_model} or $\beta$ (which controls \textit{data} heterogeneity across users) in Fig.~\ref{logistic_10_20_epochs_data}. In both of these settings, \texttt{DP-SCAFFOLD-warm} performs consistently better.
    \item \textbf{FEMNIST data.} In Fig.~\ref{femnist_10_20_epochs_accuracy}, we put in perspective the accuracy observed with $K=50$ (see Fig.~\ref{femnist_10_epochs_heterogene}) with the one observed with $K=100$. We also show the evolution of the gradient dissimilarity in Fig.~\ref{femnist_10_20_epochs_diss}. These results on real data again show the superior performance of \texttt{DP-SCAFFOLD-warm}, consistently with our observations on simulated data. % which demonstrates coherence over the performance on \texttt{DP-SCAFFOLD-warm} for real-world data.
\end{itemize}

\paragraph{Experiments with $K$ fixed and $T$ maximized.}

For this experiment conducted on simulated data, we keep the same privacy budget as described in Section~\ref{sec:experiments} as well as the same values for $l$ and $s$. Given some values for $\sigma_g$ and $K$, we calculate the maximal value of $T$ such that the privacy guarantee is still maintained in the output after $T$ communication rounds. We compute in Table~\ref{table_experiments_k_fixed} the test accuracy obtained after these iterations (average over 3 random runs) for a low heterogeneity setting $(\alpha, \beta)=(0,0)$ and a strong heterogeneity setting $(\alpha, \beta)=(5,5)$. Our results show that, given a constraint on $T$, $K$ (and thus $\sigma_g$), \texttt{DP-SCAFFOLD-warm} is even more efficient when the heterogeneity is high. Our analysis also highlights the trade-off between $T$ and $K$ (which relates to hardware and communication constraints in real deployments) to achieve some given performance. For example, we show that under high heterogeneity, we obtain roughly the same accuracy if we run \texttt{DP-SCAFFOLD-warm} with $(T,K)=(266,5)$ or $(T,K)=(182,20)$ (in \textcolor{blue!75!black}{blue}), as well as $(T,K)=(62,20)$ or $(T,K)=(42,80)$ (in \textcolor{red!75!black}{red}). In practical deployments, $T$ is often the bottleneck, so smaller $T$ and larger $K$ are often preferred. Note also that we observe a threshold due to a DP noise when $(\sigma_g,K)=(40,20)$, which leads to the same performance as the setting $(\sigma_g,K)=(20,5)$ (in \textcolor{brown!75!black}{brown}).

\begin{table}[h!]
\caption{Test Accuracy for \texttt{DP-SCAFFOLD-warm} with $T$ maximized (simulated data, $\epsilon=1.5$)}
\label{table_experiments_k_fixed}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c||c|c|c|c|c|c|}
\hline
\textbf{$\sigma_g$}  &$(\alpha, \beta)$ &\multicolumn{2}{c|}{$K=5$} & \multicolumn{2}{c|}{$K=20$} & \multicolumn{2}{c|}{$K=80$} \\
\hline
\multirow{2}{*}{15} & \textcolor{green!50!black}{(0,0)} &  48.93\% $\mp$ 0.73 & \multirow{2}{*}{$T= 266$}
                            &  42.46\% $\mp$ 0.25 & \multirow{2}{*}{$T= 62$}
                            &  24.11\% $\mp$ 1.75 & \multirow{2}{*}{$T= 14$}\\
   & \textcolor{orange!75!black}{(5,5)} &  \textcolor{blue!75!black}{\textbf{58.02}}\% $\mp$ 3.16 & &  \textcolor{red!75!black}{\textbf{47.76}}\% $\mp$ 0.09 & &  \textbf{28.14}\% $\mp$ 2.80 &  \\
\hline
\multirow{2}{*}{20} & \textcolor{green!50!black}{(0,0)} &  51.83\% $\mp$ 0.95 & \multirow{2}{*}{$T= 480$}
                            &  46.48\% $\mp$ 1.67 & \multirow{2}{*}{$T= 114$}
                            &  34.70\% $\mp$ 1.25 & \multirow{2}{*}{$T= 26$}\\
   & \textcolor{orange!75!black}{(5,5)} &  \textcolor{brown!75!black}{\textbf{64.97}}\% $\mp$ 1.34 & &  \textbf{55.34}\% $\mp$ 1.17 & &  \textbf{37.41}\% $\mp$ 3.41 &  \\
\hline
\multirow{2}{*}{25} &\textcolor{green!50!black}{(0,0)}  &  \multirow{2}{*}{\textit{Not done}} & \multirow{2}{*}{$T= 758$}  
                            &  49.72\% $\mp$ 0.14 & \multirow{2}{*}{$T= 182$}  
                            &  39.39\% $\mp$ 0.15 & \multirow{2}{*}{$T= 42$}\\
   & \textcolor{orange!75!black}{(5,5)} &   & &  \textcolor{blue!75!black}{\textbf{59.74}}\% $\mp$ 1.63 & &  \textcolor{red!75!black}{\textbf{44.02}}\% $\mp$ 1.36 &  \\
\hline
\multirow{2}{*}{40} &\textcolor{green!50!black}{(0,0)}  &  \multirow{2}{*}{\textit{Not done}} & \multirow{2}{*}{$T= 1972$}  
                            & 51.83\% $\mp$ 0.81  & \multirow{2}{*}{$T= 480$}  
                            &  45.23\% $\mp$ 1.33 & \multirow{2}{*}{$T= 114$}\\
   & \textcolor{orange!75!black}{(5,5)} &   & &  \textcolor{brown!75!black}{\textbf{62.11}}\% $\mp$ 1.83 & & \textbf{54.49}\% $\mp$ 1.61  &  \\
\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_accuracy_k_10.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_accuracy_k_20.pdf}
    \caption{Test Accuracy on simulated data with $(1.5,2.10^{-6})$-DP. First row: $K=50$; Second row: $K=100$.}
    \label{logistic_10_20_epochs_accuracy}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_diss_k_10.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_diss_k_20.pdf}
    \caption{Train Grad. Diss. on simulated data with $(1.5,2.10^{-6})$-DP. First row: $K=50$; Second row: $K=100$.}
    \label{logistic_10_20_epochs_diss}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_loss_k_10_model.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_loss_k_20_model.pdf}
    \caption{Model Heterogeneity : Train Loss on simulated data with $(1.5,2.10^{-6})$-DP ($K=50$ and $K=100$)}
    \label{logistic_10_20_epochs_model}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_loss_k_10_data.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/logistic_loss_k_20_data.pdf}
    \caption{Data Heterogeneity : Train Loss on simulated data with $(1.5,2.10^{-6})$-DP ($K=50$ and $K=100$)}
    \label{logistic_10_20_epochs_data}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/femnist_accuracy_k_10.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/femnist_accuracy_k_20.pdf}
    \caption{Test Accuracy on FEMNIST data with $(4.5,10^{-5})$-DP. First row: $K=50$; Second row: $K=100$.}
    \label{femnist_10_20_epochs_accuracy}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/femnist_diss_k_10.pdf} \\
\vspace{0.6em}
    \includegraphics[width=\linewidth]{Paper_AISTATS/figures_main_aistats/femnist_diss_k_20.pdf}
    \caption{Train Grad. Diss. on FEMNIST data with $(4.5,10^{-5})$-DP. First row: $K=50$; Second row: $K=100$.}
    \label{femnist_10_20_epochs_diss}
\end{figure*}




==> brouillon.tex <==
\paragraph{Experiments with $T$ fixed and $K$ growing.} In this part, we aim to highlight the impact of $K$ in the performance of the DP versions of \texttt{SCAFFOLD} and \texttt{FedAvg}. We fix $T=400$ and compute the metrics for simulated data (Fig.~\ref{logistic_all_epochs}, $\gamma\in \{0\%, 10\%, 100\%\}$) and for FEMNIST data (Fig.~\ref{femnist_all_epochs}, $(\alpha, \beta) \in \{(0,0), (1,1), (5,5)\}$) with $K\in \{5, 20, 40\}$, while keeping the same privacy budget (average over 3 random runs). Remark that the value of $\sigma_g$ is lower for \texttt{DP-SCAFFOLD-warm} than \texttt{DP-FedAvg}, due to the saving of the first rounds for the warm-start version (no model is trained yet). Local learning rate factor $\eta_0$ was carefully tuned for each value of $K$ (5-fold cross-validation). Our results show that \texttt{DP-SCAFFOLD-warm} does not suffer from an increasing value of $K$ (on the contrary, \texttt{DP-FedAvg} is more fluctuating as $K$ grows) and consistently outperforms \texttt{DP-FedAvg}. However, we do not observe a clear improvement of the precision of the model trained with \texttt{DP-SCAFFOLD-warm} as $K$ grows.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper-AISTATS/figures_main_aistats/test_accuracy_femnist_all_K.pdf}
    \caption{Test Accuracy on FEMNIST data with $(4.5,10^{-5})$-DP for $T=400$.}
    \label{femnist_all_epochs}
\end{figure*}

\newpage

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{Paper-AISTATS/figures_main_aistats/test_accuracy_femnist_all_K.pdf} \\
    % \caption{Train Loss on simulated data (10 local epochs)}
    % \label{logistic_10_epochs_heterogene_all}
% \end{figure*}
% \begin{figure*}[h!]
%     \centering
\vspace{0.6em}
    \includegraphics[width=0.8\linewidth]{Paper-AISTATS/figures_main_aistats/train_loss_log_all_K.pdf}
    \caption{Metrics on simulated data with $(1.5,2.10^{-6})$-DP for $T=400$. First row: Accuracy; Second row: Loss.}
    \label{logistic_all_epochs}
\end{figure*}


\paragraph{Experiments with .}

Given some values for $\sigma_g$ and $K$, we calculate the maximal value of $T$ such that the privacy guarantee is still maintained in the output after $T$ communication rounds. We compute in Table~\ref{table_experiments_k_fixed} the test accuracy obtained after these iterations (average over 3 random runs) for a low heterogeneity setting $(\alpha, \beta)=(0,0)$ and a strong heterogeneity setting $(\alpha, \beta)=(5,5)$. Our results show that, given a constraint on $T$, $K$ (and thus $\sigma_g$), \texttt{DP-SCAFFOLD-warm} is even more efficient when the heterogeneity is high. Our analysis also highlights the trade-off between $T$ and $K$ (which relates to hardware and communication constraints in real deployments) to achieve some given performance. For example, we show that under high heterogeneity, we obtain roughly the same accuracy if we run \texttt{DP-SCAFFOLD-warm} with $(T,K)=(266,5)$ or $(T,K)=(182,20)$ (in \textcolor{blue!75!black}{blue}), as well as $(T,K)=(62,20)$ or $(T,K)=(42,80)$ (in \textcolor{red!75!black}{red}). In practical deployments, $T$ is often the bottleneck, so smaller $T$ and larger $K$ are often preferred. Note also that we observe a threshold due to a DP noise when $(\sigma_g,K)=(40,20)$, which leads to similar performance as the setting $(\sigma_g,K)=(20,5)$ (in \textcolor{brown!75!black}{brown}). For our experiments, we did not take into account the communication rounds from the warm-start ($4/l=20$ rounds) to compute $T$. 

\begin{table}[h!]
\caption{Test accuracy for \texttt{DP-SCAFFOLD-warm} with $T$ maximized (simulated data, $\epsilon=1.5$)}
\label{table_experiments_k_fixed}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c||c|c|c|c|c|c|}
\hline
\textbf{$\sigma_g$}  &$(\alpha, \beta)$ &\multicolumn{2}{c|}{$K=5$} & \multicolumn{2}{c|}{$K=20$} & \multicolumn{2}{c|}{$K=80$} \\
\hline
\multirow{2}{*}{15} & \textcolor{green!50!black}{(0,0)} &  48.93\% $\mp$ 0.73 & \multirow{2}{*}{$T= 266$}
                            &  42.46\% $\mp$ 0.25 & \multirow{2}{*}{$T= 62$}
                            &  24.11\% $\mp$ 1.75 & \multirow{2}{*}{$T= 14$}\\
   & \textcolor{orange!75!black}{(5,5)} &  \textcolor{blue!75!black}{\textbf{58.02}}\% $\mp$ 3.16 & &  \textcolor{red!75!black}{\textbf{47.76}}\% $\mp$ 0.09 & &  \textbf{28.14}\% $\mp$ 2.80 &  \\
\hline
\multirow{2}{*}{20} & \textcolor{green!50!black}{(0,0)} &  51.83\% $\mp$ 0.95 & \multirow{2}{*}{$T= 480$}
                            &  46.48\% $\mp$ 1.67 & \multirow{2}{*}{$T= 114$}
                            &  34.70\% $\mp$ 1.25 & \multirow{2}{*}{$T= 26$}\\
   & \textcolor{orange!75!black}{(5,5)} &  \textcolor{brown!75!black}{\textbf{64.97}}\% $\mp$ 1.34 & &  \textbf{55.34}\% $\mp$ 1.17 & &  \textbf{37.41}\% $\mp$ 3.41 &  \\
\hline
\multirow{2}{*}{25} &\textcolor{green!50!black}{(0,0)}  &  \multirow{2}{*}{\textit{Not done}} & \multirow{2}{*}{$T= 758$}  
                            &  49.72\% $\mp$ 0.14 & \multirow{2}{*}{$T= 182$}  
                            &  39.39\% $\mp$ 0.15 & \multirow{2}{*}{$T= 42$}\\
   & \textcolor{orange!75!black}{(5,5)} &   & &  \textcolor{blue!75!black}{\textbf{59.74}}\% $\mp$ 1.63 & &  \textcolor{red!75!black}{\textbf{44.02}}\% $\mp$ 1.36 &  \\
\hline
\multirow{2}{*}{40} &\textcolor{green!50!black}{(0,0)}  &  \multirow{2}{*}{\textit{Not done}} & \multirow{2}{*}{$T= 1972$}  
                            & 51.83\% $\mp$ 0.81  & \multirow{2}{*}{$T= 480$}  
                            &  45.23\% $\mp$ 1.33 & \multirow{2}{*}{$T= 114$}\\
   & \textcolor{orange!75!black}{(5,5)} &   & &  \textcolor{brown!75!black}{\textbf{62.11}}\% $\mp$ 1.83 & & \textbf{54.49}\% $\mp$ 1.61  &  \\
\hline
\end{tabular}
}
\end{center}
\end{table}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

